Molecular-driven Foundation Model for Oncologic Pathology

Foundation models are reshaping computational pathology by enabling transfer learning, where models pre-trained on vast datasets can be adapted for downstream diagnostic, prognostic, and therapeutic response tasks. Despite these advances, foundation models are still limited in their ability to encode the entire gigapixel whole-slide images without additional training and often lack complementary multimodal data. Here, we introduce Threads, a slide-level foundation model capable of generating universal representations of whole-slide images of any size. Threads was pre-trained using a multimodal learning approach on a diverse cohort of 47,171 hematoxylin and eosin (H&E)-stained tissue sections, paired with corresponding genomic and transcriptomic profiles - the largest such paired dataset to be used for foundation model development to date. This unique training paradigm enables Threads to capture the tissue's underlying molecular composition, yielding powerful representations applicable to a wide array of downstream tasks. In extensive benchmarking across 54 oncology tasks, including clinical subtyping, grading, mutation prediction, immunohistochemistry status determination, treatment response prediction, and survival prediction, Threads outperformed all baselines while demonstrating remarkable generalizability and label efficiency. It is particularly well suited for predicting rare events, further emphasizing its clinical utility. We intend to make the model publicly available for the broader community.

==> figures/main/main_figs.tex <==

% Figure 1: Study overview

Panel A: Pretraining data overview
- Tissue site distribution as vertical bar plot (use the highest level of the oncotree classification)
- Distinguish the different sources (TCGA, GTEX, Fusion, OP)
- Show if cancer or non-cancer 

==> Extended Data Figure:
- Show the diversity in mutation in OP?

==> Extended Data Figure:
- Visualize multiple attention heads (transformer heads?) in the model. Similar to MADELEINE Suppl figure. Can be done with patch over for fine-grained mapping. 

Panel B: Method overview  => need to finalize the model overview 
- take inspiration from Tangle/Madeleine
- More high-level 

Panel C: Overview of downstream tasks
- Prediction:
   - Cancer subtyping prediction
   - Cancer grading prediction
   - Mutation status prediction 
   - IHC status prediction 
   - Gene fusion status prediction 
   - Treatment response prediction
   - Survival prediction 

- Retrieval:
   - BRACS 
   - eBRAINS 
   - 

- Slide retrieval 
- Cross-modal retrieval 
- Molecular prompting 

Panel D: Visualize a UMAP of: ==> OK
- All the slide embeddings (from CPTAC or even training slides)
- Their corresponding molecular embeddings
- Draw a straight line between pairs of S+E in the embedding space
- Include a bunch of zoom showing different diseases and/or the diversity within each disease. 

==> Extended Data Figure:
- Additional results here. 
- Could be downstream datasets, such as CPTAC 

Panel E: Scaling laws in molecular-driven pretraining ==> OK
- ABMIL --> MH-ABMIL --> ViT
- TCGA --> TCGA+OP --> TCGA+OP+Fusion --> TCGA+OP+Fusion+GTEX

% Figure 2: Performance (few-shot, all in mutation + grading + subtyping)

Panel A: Tumor subtyping with All
- Bar plot with multiple tasks (similar to UNI, fig 2.f)
- Baselines: Mean, HIPT, GigaPath, CHIEF?, TANGLE, MADELEINE 

Panel B,C,D,E: Few-shot
- select 4 tasks for which we get good performance to compare against the same bad boys 

Panel F: Mutation prediction

% Figure 3: Treatment response for classification, clustering and stratification (KM)
- GBM 
- Ovarian 
- CPTAC (replace treatment response by survival)

Panel B: UMAP of TNBC

Panel C: CPTAC with a lot of death stratification (LUAD?, LUSC?, ccRCC?)
- Clustering of all cases based on slide embedding 
- Then KM for different subgroups using survival data

Panel D: Ovarian stratification
- Clustering of TNBC cases based on slide embedding 
- Then KM for different subgroups using survival data

Panel D: GBM stratification
- Clustering of GBM cases based on slide embedding 
- Then KM for different subgroups using survival data

Panel F: Treatment response prediction 
- all bar plots with results against baselines

Panel G: UMAP response viz
- UMAP of the different slide embeddings labeled by response (or other markers if available). Show some stratification 


% Figure 4: Retrieval, prompting, and reader study
Panel A: mAP for retrieval in BRACS, eBRAINS and OP? Biopsy dataset? against baselines. Can include Tangle and Madeleine as "disease-specific models"

Panel B: TNBC reader study 
- Given a reference, answer if the reference and retrieved share:
- A lot of morphological similarities 
- Some morphological similarities
- Little morphological similarities 
- No morphological similarities 
- + Adding why
- GigaPath, Random and Threads

Panel C: Prompting -- Still TBD -- should it be another figure?
- What is the morphology of TP53-mutated profiles?

% Additional ideas (panel-level)






==> tables/archived/downstream_performance.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on MGB-Breast tasks.} Best in \textbf{bold}, second best is \underline{underlined}. All tasks evaluated using AUROC, with mean and standard error reported over 5-fold cross-validation. ER: \textit{estrogen receptor}; PR: \textit{progesterone receptor}; HER2: \textit{human epidermal growth factor receptor 2.}}
\begin{tabular}{ll|cccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{4}{c}{Tasks} \\ 
\cmidrule(lr){3-6}
& & Subtype ($\uparrow$) (n=1264) & ER ($\uparrow$) (n=874) & PR ($\uparrow$) (n=874) & HER2 ($\uparrow$) (n=816) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.868 ± 0.013 & 0.691 ± 0.012 & 0.670 ± 0.015 & 0.588 ± 0.029 \\
& \prism\cite{} & \textbf{0.982 ± 0.003} & \underline{0.780 ± 0.020} & \underline{0.738 ± 0.020} & \textbf{0.708 ± 0.026} \\
& \gigapath\cite{} & 0.842 ± 0.014 & 0.694 ± 0.018 & 0.687 ± 0.015 & 0.567 ± 0.030 \\
& $\ours$ & \underline{0.922 ± 0.006} & \textbf{0.784 ± 0.017} & \textbf{0.741 ± 0.019} & \underline{0.701 ± 0.027} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.973 ± 0.005 & \underline{0.728 ± 0.026} & \underline{0.720 ± 0.012} & 0.656 ± 0.042 \\
& \prism\cite{} & \textbf{0.985 ± 0.002} & 0.727 ± 0.022 & 0.639 ± 0.001 & \textbf{0.710 ± 0.021} \\
& \gigapath\cite{} & 0.974 ± 0.003 & 0.709 ± 0.014 & 0.689 ± 0.020 & 0.596 ± 0.010 \\
& $\ours$ & \underline{0.983 ± 0.004} & \textbf{0.784 ± 0.016} & \textbf{0.748 ± 0.021} & \underline{0.694 ± 0.031} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.983 ± 0.004 & 0.720 ± 0.025 & 0.690 ± 0.007 & 0.622 ± 0.012 \\
& \gigapath\cite{} & \textbf{0.988 ± 0.001} & \underline{0.756 ± 0.017} & \underline{0.728 ± 0.015} & \underline{0.682 ± 0.021} \\
& $\ours$ & \underline{0.985 ± 0.003} & \textbf{0.774 ± 0.026} & \textbf{0.745 ± 0.019} & \textbf{0.693 ± 0.037} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_mgb_brca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on MGB-Lung tasks.} Best in \textbf{bold}, second best is \underline{underlined}. All tasks evaluated using AUROC, with mean and standard error reported over 5-fold cross-validation. TTF-1: \textit{Thyroid Transcription Factor-1}; P40: \textit{Delta NP63}; P63: \textit{Tumor protein 63}; CDX-2: \textit{Caudal Type Homeobox 2}; CK5-6: \textit{Cytokeratin 5/6}
}
\scalebox{0.65}{
\begin{tabular}{ll|ccccccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{7}{c}{Tasks} \\ 
\cmidrule(lr){3-9}
& & Subtype ($\uparrow$) (n=1939) & TTF-1 ($\uparrow$) (n=488) & P40 ($\uparrow$) (n=185) & P63 ($\uparrow$) (n=153) & Napsina ($\uparrow$) (n=126) & CDX-2 ($\uparrow$) (n=79) & CK5-6 ($\uparrow$) (n=58) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.830 ± 0.007 & 0.699 ± 0.027 & 0.637 ± 0.021 & 0.681 ± 0.052 & 0.669 ± 0.037 & 0.628 ± 0.081 & 0.748 ± 0.072 \\
& \prism\cite{} & \textbf{0.988 ± 0.002} & \textbf{0.890 ± 0.012} & \underline{0.885 ± 0.029} & \underline{0.793 ± 0.052} & \underline{0.786 ± 0.021} & \textbf{0.720 ± 0.061} & \underline{0.890 ± 0.026} \\
& \gigapath\cite{} & 0.754 ± 0.007 & 0.629 ± 0.022 & 0.401 ± 0.007 & 0.633 ± 0.036 & 0.605 ± 0.029 & 0.452 ± 0.047 & 0.661 ± 0.090 \\
& $\ours$ & \underline{0.983 ± 0.002} & \underline{0.864 ± 0.020} & \textbf{0.897 ± 0.025} & \textbf{0.846 ± 0.026} & \textbf{0.796 ± 0.010} & \underline{0.691 ± 0.058} & \textbf{0.928 ± 0.017} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.969 ± 0.003 & 0.836 ± 0.009 & \underline{0.867 ± 0.015} & 0.748 ± 0.034 & \underline{0.773 ± 0.044} & 0.588 ± 0.073 & \underline{0.884 ± 0.047} \\
& \prism\cite{} & \underline{0.978 ± 0.005} & \underline{0.859 ± 0.014} & 0.863 ± 0.017 & \underline{0.810 ± 0.013} & 0.704 ± 0.015 & \textbf{0.738 ± 0.032} & 0.877 ± 0.022 \\
& \gigapath\cite{} & 0.957 ± 0.003 & 0.838 ± 0.013 & 0.699 ± 0.022 & 0.653 ± 0.033 & 0.630 ± 0.040 & 0.485 ± 0.093 & 0.676 ± 0.067 \\
& $\ours$ & \textbf{0.982 ± 0.004} & \textbf{0.895 ± 0.011} & \textbf{0.898 ± 0.027} & \textbf{0.879 ± 0.020} & \textbf{0.817 ± 0.033} & \underline{0.725 ± 0.062} & \textbf{0.933 ± 0.026} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.980 ± 0.003 & 0.869 ± 0.014 & \underline{0.855 ± 0.032} & \underline{0.817 ± 0.034} & \underline{0.817 ± 0.021} & \underline{0.666 ± 0.058} & \textbf{0.883 ± 0.035} \\
& \gigapath\cite{} & \underline{0.986 ± 0.004} & \underline{0.890 ± 0.007} & 0.620 ± 0.050 & 0.682 ± 0.020 & 0.688 ± 0.029 & 0.496 ± 0.048 & 0.537 ± 0.102 \\
& $\ours$ & \textbf{0.988 ± 0.001} & \textbf{0.892 ± 0.008} & \textbf{0.893 ± 0.026} & \textbf{0.862 ± 0.022} & \textbf{0.820 ± 0.017} & \textbf{0.724 ± 0.042} & \underline{0.874 ± 0.032} \\
\midrule
\bottomrule
\end{tabular}
}
\label{tab:normal_mgb_lung}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on BCNB\cite{xu2021predicting} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level tasks evaluated using AUROC, with mean and standard error reported over 5-fold cross-validation. ER: \textit{estrogen receptor}; PR: \textit{progesterone receptor}; HER2: \textit{human epidermal growth factor receptor 2.}}
\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & ER ($\uparrow$) (n=1058) & PR ($\uparrow$) (n=1058) & HER2 ($\uparrow$) (n=1058) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.833 ± 0.011 & 0.780 ± 0.024 & 0.692 ± 0.018 \\
& \prism\cite{} & \underline{0.843 ± 0.013} & \underline{0.792 ± 0.014} & \underline{0.734 ± 0.012} \\
& \gigapath\cite{} & 0.800 ± 0.017 & 0.755 ± 0.019 & 0.673 ± 0.021 \\
& $\ours$ & \textbf{0.896 ± 0.010} & \textbf{0.834 ± 0.017} & \textbf{0.753 ± 0.012} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.889 ± 0.010 & 0.810 ± 0.022 & \underline{0.737 ± 0.013} \\
& \prism\cite{} & \underline{0.892 ± 0.014} & \underline{0.816 ± 0.019} & 0.711 ± 0.010 \\
& \gigapath\cite{} & 0.886 ± 0.016 & 0.810 ± 0.013 & 0.701 ± 0.016 \\
& $\ours$ & \textbf{0.921 ± 0.009} & \textbf{0.837 ± 0.020} & \textbf{0.765 ± 0.008} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.880 ± 0.011 & 0.810 ± 0.011 & 0.736 ± 0.019 \\
& \gigapath\cite{} & \textbf{0.930 ± 0.009} & \textbf{0.858 ± 0.015} & \underline{0.762 ± 0.018} \\
& $\ours$ & \underline{0.921 ± 0.013} & \underline{0.840 ± 0.015} & \textbf{0.788 ± 0.006} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_bcnb}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on MUT-HET-RCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level tasks evaluated using AUROC, with mean and standard error reported over 5-fold cross-validation.}
\scalebox{0.9}{
\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & BAP1 Mutation ($\uparrow$) (n=1291) & PBRM1 Mutation ($\uparrow$) (n=1291) & SETD2 Mutation ($\uparrow$) (n=1291) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.828 ± 0.022} & 0.673 ± 0.006 & \textbf{0.704 ± 0.009} \\
& \prism\cite{} & 0.827 ± 0.016 & \underline{0.701 ± 0.008} & 0.683 ± 0.015 \\
& \gigapath\cite{} & 0.823 ± 0.018 & 0.682 ± 0.004 & \underline{0.695 ± 0.015} \\
& $\ours$ & \textbf{0.851 ± 0.010} & \textbf{0.760 ± 0.003} & 0.689 ± 0.012 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.846 ± 0.011 & 0.781 ± 0.004 & 0.728 ± 0.011 \\
& \prism\cite{} & 0.848 ± 0.017 & \underline{0.798 ± 0.008} & \underline{0.733 ± 0.009} \\
& \gigapath\cite{} & \underline{0.858 ± 0.007} & 0.798 ± 0.003 & 0.712 ± 0.012 \\
& $\ours$ & \textbf{0.873 ± 0.006} & \textbf{0.826 ± 0.003} & \textbf{0.756 ± 0.009} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.884 ± 0.008 & 0.783 ± 0.009 & 0.717 ± 0.009 \\
& \gigapath\cite{} & \textbf{0.905 ± 0.004} & \textbf{0.820 ± 0.014} & \underline{0.728 ± 0.009} \\
& $\ours$ & \underline{0.896 ± 0.007} & \underline{0.817 ± 0.008} & \textbf{0.741 ± 0.007} \\
\midrule
\bottomrule
\end{tabular}
}
\label{tab:normal_mut-het-rcc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on IMP\cite{neto2024interpretable}.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Grade}: Slide-level tasks evaluated using balanced accuracy, with mean and 95\% CI reported over 100 bootstraps of a single fold.}
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Grade ($\uparrow$) (n=4437) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.791 ± TBD (0.000) \\
& \prism\cite{} & nan ± TBD (nan) \\
& \gigapath\cite{} & \textbf{0.839 ± TBD (0.000)} \\
& $\ours$ & \underline{0.835 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.907 ± TBD (0.000) \\
& \prism\cite{} & nan ± TBD (nan) \\
& \gigapath\cite{} & \underline{0.928 ± TBD (0.000)} \\
& $\ours$ & \textbf{0.933 ± TBD (0.000)} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.949 ± TBD (0.000)} \\
& \gigapath\cite{} & \textbf{0.969 ± TBD (0.000)} \\
& $\ours$ & 0.946 ± TBD (0.000) \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_imp}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on PANDA\cite{bulten2022artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level task evaluated using quadratic weighted kappa, mean and 95\% CI reported over 100 bootstraps of a single fold.}
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & ISUP Grade ($\uparrow$) (n=9555) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.701 ± TBD (0.000) \\
& \prism\cite{} & \underline{0.809 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.465 ± TBD (0.000) \\
& $\ours$ & \textbf{0.814 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.844 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.919 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.872 ± TBD (0.000) \\
& $\ours$ & \underline{0.915 ± TBD (0.000)} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.932 ± TBD (0.000) \\
& \gigapath\cite{} & \textbf{0.954 ± TBD (0.000)} \\
& $\ours$ & \underline{0.933 ± TBD (0.000)} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_panda}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-BRCA\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo.}
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & PIK3CA Mutation ($\uparrow$) (n=103) & TP53 Mutation ($\uparrow$) (n=103) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.602 ± 0.015} & 0.783 ± 0.014 \\
& \prism\cite{} & 0.578 ± 0.016 & \underline{0.839 ± 0.011} \\
& \gigapath\cite{} & 0.546 ± 0.018 & 0.743 ± 0.014 \\
& $\ours$ & \textbf{0.637 ± 0.014} & \textbf{0.873 ± 0.012} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.512 ± 0.017 & \underline{0.796 ± 0.011} \\
& \prism\cite{} & \textbf{0.575 ± 0.014} & 0.787 ± 0.013 \\
& \gigapath\cite{} & 0.536 ± 0.018 & 0.742 ± 0.013 \\
& $\ours$ & \underline{0.571 ± 0.017} & \textbf{0.876 ± 0.012} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.522 ± 0.015 & \underline{0.791 ± 0.013} \\
& \gigapath\cite{} & \underline{0.561 ± 0.016} & 0.768 ± 0.014 \\
& $\ours$ & \textbf{0.605 ± 0.016} & \textbf{0.846 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_brca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-CCRCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BAP1, PBRM1 mutation}: patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: patient-level survival task evaluated using c-index, mean and standard error reported over 5-fold cross-validation. }
\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & BAP1 Mutation ($\uparrow$) (n=103) & PBRM1 Mutation ($\uparrow$) (n=103) & Survival ($\uparrow$) (n=0) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.723 ± 0.020 & 0.551 ± 0.018 & \textbf{} \\
& \prism\cite{} & \underline{0.729 ± 0.017} & \underline{0.593 ± 0.019} & \textbf{} \\
& \gigapath\cite{} & 0.679 ± 0.024 & 0.455 ± 0.016 & \textbf{} \\
& $\ours$ & \textbf{0.861 ± 0.009} & \textbf{0.635 ± 0.016} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.655 ± 0.016 & 0.518 ± 0.015 & \textbf{} \\
& \prism\cite{} & \underline{0.664 ± 0.022} & \underline{0.598 ± 0.019} & \textbf{} \\
& \gigapath\cite{} & 0.654 ± 0.024 & 0.497 ± 0.016 & \textbf{} \\
& $\ours$ & \textbf{0.809 ± 0.014} & \textbf{0.668 ± 0.016} & \textbf{} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.724 ± 0.019} & \underline{0.580 ± 0.019} & \textbf{} \\
& \gigapath\cite{} & 0.721 ± 0.019 & 0.484 ± 0.015 & \textbf{} \\
& $\ours$ & \textbf{0.787 ± 0.016} & \textbf{0.631 ± 0.016} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_ccrcc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-COAD\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo.}
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & KRAS Mutation ($\uparrow$) (n=94) & TP53 Mutation ($\uparrow$) (n=94) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \textbf{0.655 ± 0.015} & \underline{0.657 ± 0.019} \\
& \prism\cite{} & 0.472 ± 0.016 & 0.581 ± 0.020 \\
& \gigapath\cite{} & 0.582 ± 0.015 & 0.633 ± 0.019 \\
& $\ours$ & \underline{0.621 ± 0.015} & \textbf{0.805 ± 0.014} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \textbf{0.742 ± 0.016} & \underline{0.690 ± 0.018} \\
& \prism\cite{} & 0.554 ± 0.015 & 0.578 ± 0.019 \\
& \gigapath\cite{} & 0.647 ± 0.014 & 0.648 ± 0.016 \\
& $\ours$ & \underline{0.704 ± 0.014} & \textbf{0.742 ± 0.016} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.628 ± 0.017} & \underline{0.747 ± 0.014} \\
& \gigapath\cite{} & 0.596 ± 0.014 & 0.635 ± 0.016 \\
& $\ours$ & \textbf{0.665 ± 0.016} & \textbf{0.785 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_coad}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-GBM\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Patient-level classification tasks evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo.}
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & EGFR Mutation ($\uparrow$) (n=99) & TP53 Mutation ($\uparrow$) (n=99) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.654 ± 0.014} & 0.738 ± 0.017 \\
& \prism\cite{} & 0.586 ± 0.016 & \textbf{0.770 ± 0.017} \\
& \gigapath\cite{} & 0.618 ± 0.014 & 0.622 ± 0.019 \\
& $\ours$ & \textbf{0.757 ± 0.015} & \underline{0.744 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.639 ± 0.014} & 0.828 ± 0.014 \\
& \prism\cite{} & 0.618 ± 0.015 & \textbf{0.858 ± 0.015} \\
& \gigapath\cite{} & 0.633 ± 0.017 & 0.773 ± 0.014 \\
& $\ours$ & \textbf{0.782 ± 0.011} & \underline{0.842 ± 0.013} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.711 ± 0.015} & \underline{0.835 ± 0.014} \\
& \gigapath\cite{} & 0.604 ± 0.015 & 0.643 ± 0.016 \\
& $\ours$ & \textbf{0.791 ± 0.009} & \textbf{0.867 ± 0.012} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_gbm}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-HNSC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{CASP8 Mutation}: patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & CASP8 Mutation ($\uparrow$) (n=107) & Survival ($\uparrow$) (n=0) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.675 ± 0.022} & \textbf{} \\
& \prism\cite{} & 0.674 ± 0.025 & \textbf{} \\
& \gigapath\cite{} & 0.602 ± 0.027 & \textbf{} \\
& $\ours$ & \textbf{0.778 ± 0.018} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.614 ± 0.028} & \textbf{} \\
& \prism\cite{} & 0.601 ± 0.027 & \textbf{} \\
& \gigapath\cite{} & 0.501 ± 0.023 & \textbf{} \\
& $\ours$ & \textbf{0.754 ± 0.019} & \textbf{} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.657 ± 0.033} & \textbf{} \\
& \gigapath\cite{} & 0.614 ± 0.027 & \textbf{} \\
& $\ours$ & \textbf{0.733 ± 0.025} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_hnsc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-LSCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{KEAP1, ARID1A mutation}: patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation.}
\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & KEAP1 Mutation ($\uparrow$) (n=108) & ARID1A Mutation ($\uparrow$) (n=108) & Survival ($\uparrow$) (n=0) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \textbf{0.669 ± 0.017} & 0.521 ± 0.020 & \textbf{} \\
& \prism\cite{} & 0.456 ± 0.018 & 0.548 ± 0.023 & \textbf{} \\
& \gigapath\cite{} & 0.576 ± 0.021 & \underline{0.590 ± 0.020} & \textbf{} \\
& $\ours$ & \underline{0.646 ± 0.021} & \textbf{0.610 ± 0.027} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.574 ± 0.018 & 0.411 ± 0.020 & \textbf{} \\
& \prism\cite{} & 0.491 ± 0.018 & 0.449 ± 0.020 & \textbf{} \\
& \gigapath\cite{} & \underline{0.644 ± 0.018} & \underline{0.490 ± 0.017} & \textbf{} \\
& $\ours$ & \textbf{0.685 ± 0.019} & \textbf{0.658 ± 0.023} & \textbf{} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.470 ± 0.023 & 0.469 ± 0.027 & \textbf{} \\
& \gigapath\cite{} & \underline{0.613 ± 0.020} & \textbf{0.553 ± 0.019} & \textbf{} \\
& $\ours$ & \textbf{0.614 ± 0.017} & \underline{0.508 ± 0.023} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_lscc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-LUAD\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{EGFR, STK11, TP53 mutation}: patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation.}
\scalebox{0.8}{
\begin{tabular}{ll|cccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{4}{c}{Tasks} \\ 
\cmidrule(lr){3-6}
& & EGFR Mutation ($\uparrow$) (n=108) & STK11 Mutation ($\uparrow$) (n=108) & TP53 Mutation ($\uparrow$) (n=108) & Survival ($\uparrow$) (n=0) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.748 ± 0.017} & 0.810 ± 0.020 & 0.663 ± 0.016 & \textbf{} \\
& \prism\cite{} & 0.722 ± 0.016 & \underline{0.875 ± 0.015} & \underline{0.688 ± 0.016} & \textbf{} \\
& \gigapath\cite{} & 0.723 ± 0.018 & 0.770 ± 0.022 & 0.631 ± 0.018 & \textbf{} \\
& $\ours$ & \textbf{0.767 ± 0.014} & \textbf{0.893 ± 0.015} & \textbf{0.722 ± 0.014} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.789 ± 0.014 & 0.824 ± 0.018 & 0.682 ± 0.015 & \textbf{} \\
& \prism\cite{} & \underline{0.809 ± 0.013} & \underline{0.854 ± 0.015} & \textbf{0.756 ± 0.013} & \textbf{} \\
& \gigapath\cite{} & 0.786 ± 0.014 & 0.827 ± 0.014 & 0.733 ± 0.013 & \textbf{} \\
& $\ours$ & \textbf{0.822 ± 0.011} & \textbf{0.889 ± 0.015} & \underline{0.752 ± 0.014} & \textbf{} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.761 ± 0.016} & \underline{0.840 ± 0.015} & 0.671 ± 0.015 & \textbf{} \\
& \gigapath\cite{} & 0.732 ± 0.015 & 0.812 ± 0.017 & \underline{0.695 ± 0.017} & \textbf{} \\
& $\ours$ & \textbf{0.792 ± 0.015} & \textbf{0.895 ± 0.011} & \textbf{0.758 ± 0.013} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}
\label{tab:normal_cptac_luad}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on CPTAC-PDAC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{SMAD4 mutation}: patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & SMAD4 Mutation ($\uparrow$) (n=105) & Survival ($\uparrow$) (n=0) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.606 ± 0.021} & \textbf{} \\
& \prism\cite{} & 0.593 ± 0.023 & \textbf{} \\
& \gigapath\cite{} & 0.311 ± 0.020 & \textbf{} \\
& $\ours$ & \textbf{0.666 ± 0.022} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.576 ± 0.020} & \textbf{} \\
& \prism\cite{} & 0.523 ± 0.022 & \textbf{} \\
& \gigapath\cite{} & 0.426 ± 0.021 & \textbf{} \\
& $\ours$ & \textbf{0.578 ± 0.024} & \textbf{} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.502 ± 0.019} & \textbf{} \\
& \gigapath\cite{} & 0.331 ± 0.018 & \textbf{} \\
& $\ours$ & \textbf{0.582 ± 0.022} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_cptac_pda}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on BRACS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level classification tasks evaluated using balanced accuracy, mean and standard error reported over 5-fold cross-validation.}
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=547) & Coarse Subtype ($\uparrow$) (n=547) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.336 ± 0.019 & 0.645 ± 0.020 \\
& \prism\cite{} & \textbf{0.474 ± 0.027} & \textbf{0.726 ± 0.020} \\
& \gigapath\cite{} & 0.286 ± 0.018 & 0.575 ± 0.033 \\
& $\ours$ & \underline{0.452 ± 0.024} & \underline{0.724 ± 0.028} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.377 ± 0.036 & 0.623 ± 0.036 \\
& \prism\cite{} & \underline{0.420 ± 0.015} & \underline{0.658 ± 0.019} \\
& \gigapath\cite{} & 0.339 ± 0.018 & 0.608 ± 0.034 \\
& $\ours$ & \textbf{0.481 ± 0.015} & \textbf{0.716 ± 0.019} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \textbf{0.504 ± 0.010} & \underline{0.696 ± 0.031} \\
& \gigapath\cite{} & 0.459 ± 0.020 & 0.681 ± 0.020 \\
& $\ours$ & \underline{0.479 ± 0.022} & \textbf{0.725 ± 0.019} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_bracs}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on eBRAINS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level classification tasks evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold.}
\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=2319) & Coarse Subtype ($\uparrow$) (n=2319) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.549 ± TBD (0.000) & 0.724 ± TBD (0.000) \\
& \prism\cite{} & \underline{0.624 ± TBD (0.000)} & \underline{0.752 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.617 ± TBD (0.000) & 0.745 ± TBD (0.000) \\
& $\ours$ & \textbf{0.705 ± TBD (0.000)} & \textbf{0.839 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.693 ± TBD (0.000) & 0.874 ± TBD (0.000) \\
& \prism\cite{} & 0.714 ± TBD (0.000) & 0.872 ± TBD (0.000) \\
& \gigapath\cite{} & \underline{0.722 ± TBD (0.000)} & \underline{0.892 ± TBD (0.000)} \\
& $\ours$ & \textbf{0.741 ± TBD (0.000)} & \textbf{0.919 ± TBD (0.000)} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.722 ± TBD (0.000) & 0.882 ± TBD (0.000) \\
& \gigapath\cite{} & \textbf{0.747 ± TBD (0.000)} & \textbf{0.905 ± TBD (0.000)} \\
& $\ours$ & \underline{0.741 ± TBD (0.000)} & \underline{0.895 ± TBD (0.000)} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_ebrains}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on IMPRESS-HER2\cite{huang2023artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & pCR ($\uparrow$) (n=62) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.474 ± 0.020 \\
& \prism\cite{} & \textbf{0.667 ± 0.022} \\
& \gigapath\cite{} & 0.601 ± 0.019 \\
& $\ours$ & \underline{0.611 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.472 ± 0.019 \\
& \prism\cite{} & \textbf{0.642 ± 0.019} \\
& \gigapath\cite{} & 0.565 ± 0.022 \\
& $\ours$ & \underline{0.603 ± 0.020} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.701 ± 0.022} \\
& \gigapath\cite{} & 0.533 ± 0.018 \\
& $\ours$ & \textbf{0.709 ± 0.019} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_impress_her2}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on IMPRESS-TNBC\cite{huang2023artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & pCR ($\uparrow$) (n=64) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.570 ± 0.022 \\
& \prism\cite{} & 0.587 ± 0.021 \\
& \gigapath\cite{} & \underline{0.598 ± 0.020} \\
& $\ours$ & \textbf{0.657 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \textbf{0.652 ± 0.020} \\
& \prism\cite{} & 0.541 ± 0.017 \\
& \gigapath\cite{} & \underline{0.617 ± 0.018} \\
& $\ours$ & 0.602 ± 0.021 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \textbf{0.615 ± 0.020} \\
& \gigapath\cite{} & 0.595 ± 0.021 \\
& $\ours$ & \underline{0.604 ± 0.022} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_impress_tnbc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on OV-Bevacizumab\cite{wang2022weakly} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo.}
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=36) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.797 ± 0.026} \\
& \prism\cite{} & 0.443 ± 0.041 \\
& \gigapath\cite{} & 0.760 ± 0.028 \\
& $\ours$ & \textbf{0.857 ± 0.025} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.623 ± 0.030} \\
& \prism\cite{} & 0.433 ± 0.034 \\
& \gigapath\cite{} & 0.603 ± 0.039 \\
& $\ours$ & \textbf{0.863 ± 0.021} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.540 ± 0.033} \\
& \gigapath\cite{} & 0.457 ± 0.046 \\
& $\ours$ & \textbf{0.780 ± 0.032} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_ovarian}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on NADT Prostate\cite{wilkinson2021nascent} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo.}
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=36) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.683 ± 0.022 \\
& \prism\cite{} & \textbf{0.752 ± 0.024} \\
& \gigapath\cite{} & 0.688 ± 0.026 \\
& $\ours$ & \underline{0.725 ± 0.023} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.622 ± 0.026 \\
& \prism\cite{} & \underline{0.720 ± 0.023} \\
& \gigapath\cite{} & 0.577 ± 0.024 \\
& $\ours$ & \textbf{0.730 ± 0.022} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.583 ± 0.033} \\
& \gigapath\cite{} & 0.525 ± 0.036 \\
& $\ours$ & \textbf{0.702 ± 0.020} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_nadt}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on GBM-Treatment\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=93) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.668 ± 0.018} \\
& \prism\cite{} & 0.633 ± 0.019 \\
& \gigapath\cite{} & \textbf{0.672 ± 0.016} \\
& $\ours$ & 0.659 ± 0.018 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.703 ± 0.018} \\
& \prism\cite{} & 0.622 ± 0.022 \\
& \gigapath\cite{} & 0.618 ± 0.017 \\
& $\ours$ & \textbf{0.741 ± 0.016} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.704 ± 0.018} \\
& \gigapath\cite{} & 0.642 ± 0.017 \\
& $\ours$ & \textbf{0.707 ± 0.016} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_gbm_rt_tmz}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on Post-NAT-BRCA\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. Slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Lymphovascular Invasion ($\uparrow$) (n=53) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.568 ± 0.026 \\
& \prism\cite{} & 0.487 ± 0.024 \\
& \gigapath\cite{} & \textbf{0.627 ± 0.025} \\
& $\ours$ & \underline{0.601 ± 0.027} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.654 ± 0.022} \\
& \prism\cite{} & 0.540 ± 0.029 \\
& \gigapath\cite{} & 0.577 ± 0.024 \\
& $\ours$ & \textbf{0.701 ± 0.027} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.553 ± 0.025 \\
& \gigapath\cite{} & \underline{0.615 ± 0.025} \\
& $\ours$ & \textbf{0.662 ± 0.028} \\
\midrule
\bottomrule
\end{tabular}
\label{tab:normal_natbrca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{Performance comparison between $\ours$ and baselines on SURGEN\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BRAF Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{RAS Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{MMR Loss}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Death in 5 Years}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{5}{c}{Tasks} \\ 
\cmidrule(lr){3-7}
& & BRAF Mutation ($\uparrow$) (n=388) & RAS Mutation ($\uparrow$) (n=389) & MMR Loss ($\uparrow$) (n=389) & Death in 5 Years ($\uparrow$) (n=387) & Survival ($\uparrow$) (n=144) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.641 ± 0.020} & \underline{0.619 ± 0.020} & \underline{0.819 ± 0.026} & \underline{0.663 ± 0.023} & \textbf{} \\
& \prism\cite{} &  &  &  &  & \textbf{} \\
& \gigapath\cite{} & 0.616 ± 0.021 & 0.618 ± 0.010 & 0.779 ± 0.046 & 0.631 ± 0.024 & \textbf{} \\
& $\ours$ & \textbf{0.753 ± 0.039} & \textbf{0.649 ± 0.029} & \textbf{0.914 ± 0.019} & \textbf{0.667 ± 0.017} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.649 ± 0.025 & \underline{0.630 ± 0.028} & 0.797 ± 0.037 & \underline{0.661 ± 0.023} & \textbf{} \\
& \prism\cite{} &  &  &  &  & \textbf{} \\
& \gigapath\cite{} & \underline{0.679 ± 0.026} & 0.621 ± 0.022 & \underline{0.861 ± 0.015} & 0.633 ± 0.013 & \textbf{} \\
& $\ours$ & \textbf{0.726 ± 0.042} & \textbf{0.632 ± 0.027} & \textbf{0.910 ± 0.023} & \textbf{0.685 ± 0.017} & \textbf{} \\
\midrule
\multirow{3}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.692 ± 0.046} & \underline{0.656 ± 0.017} & \underline{0.841 ± 0.035} & \underline{0.695 ± 0.017} & \textbf{} \\
& \gigapath\cite{} &  &  &  &  & \textbf{} \\
& $\ours$ & \textbf{0.798 ± 0.031} & \textbf{0.675 ± 0.014} & \textbf{0.894 ± 0.035} & \textbf{0.733 ± 0.024} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_sr386_}
\end{table}






==> tables/archived/downstream_performance_randominit.tex <==
\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MGB Breast tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Subtype}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{ER}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{PR}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{HER2}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{4}{c}{Tasks} \\ 
\cmidrule(lr){3-6}
& & Subtype ($\uparrow$) (n=1264) & ER ($\uparrow$) (n=874) & PR ($\uparrow$) (n=874) & HER2 ($\uparrow$) (n=816) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.868 ± 0.013 & 0.691 ± 0.012 & 0.670 ± 0.015 & 0.588 ± 0.029 \\
& \prism\cite{} & \textbf{0.982 ± 0.003} & \underline{0.780 ± 0.020} & \underline{0.738 ± 0.020} & \textbf{0.708 ± 0.026} \\
& \gigapath\cite{} & 0.842 ± 0.014 & 0.694 ± 0.018 & 0.687 ± 0.015 & 0.567 ± 0.030 \\
& $\ours$ & \underline{0.922 ± 0.006} & \textbf{0.784 ± 0.017} & \textbf{0.741 ± 0.019} & \underline{0.701 ± 0.027} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.973 ± 0.005 & \underline{0.728 ± 0.026} & \underline{0.720 ± 0.012} & 0.656 ± 0.042 \\
& \prism\cite{} & \textbf{0.985 ± 0.002} & 0.727 ± 0.022 & 0.639 ± 0.001 & \textbf{0.710 ± 0.021} \\
& \gigapath\cite{} & 0.974 ± 0.003 & 0.709 ± 0.014 & 0.689 ± 0.020 & 0.596 ± 0.010 \\
& $\ours$ & \underline{0.983 ± 0.004} & \textbf{0.784 ± 0.016} & \textbf{0.748 ± 0.021} & \underline{0.694 ± 0.031} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.983 ± 0.004 & 0.720 ± 0.025 & 0.690 ± 0.007 & 0.622 ± 0.012 \\
& \gigapath\cite{} & \textbf{0.988 ± 0.001} & 0.756 ± 0.017 & 0.728 ± 0.015 & 0.682 ± 0.021 \\
& $\ours$ Random Init & \underline{0.985 ± 0.003} & \textbf{0.780 ± 0.024} & \textbf{0.757 ± 0.016} & \textbf{0.701 ± 0.040} \\
& $\ours$ & 0.985 ± 0.003 & \underline{0.774 ± 0.026} & \underline{0.745 ± 0.019} & \underline{0.693 ± 0.037} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mgb_brca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MGB Lung tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Subtype}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{TTF-1}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{P40}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{P63}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Napsina}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{CDX-2}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{CK5-6}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccccccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{7}{c}{Tasks} \\ 
\cmidrule(lr){3-9}
& & Subtype ($\uparrow$) (n=1939) & TTF-1 ($\uparrow$) (n=488) & P40 ($\uparrow$) (n=185) & P63 ($\uparrow$) (n=153) & Napsina ($\uparrow$) (n=126) & CDX-2 ($\uparrow$) (n=79) & CK5-6 ($\uparrow$) (n=58) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.830 ± 0.007 & 0.699 ± 0.027 & 0.637 ± 0.021 & 0.681 ± 0.052 & 0.669 ± 0.037 & 0.628 ± 0.081 & 0.748 ± 0.072 \\
& \prism\cite{} & \textbf{0.988 ± 0.002} & \textbf{0.890 ± 0.012} & \underline{0.885 ± 0.029} & \underline{0.793 ± 0.052} & \underline{0.786 ± 0.021} & \textbf{0.720 ± 0.061} & \underline{0.890 ± 0.026} \\
& \gigapath\cite{} & 0.754 ± 0.007 & 0.629 ± 0.022 & 0.401 ± 0.007 & 0.633 ± 0.036 & 0.605 ± 0.029 & 0.452 ± 0.047 & 0.661 ± 0.090 \\
& $\ours$ & \underline{0.983 ± 0.002} & \underline{0.864 ± 0.020} & \textbf{0.897 ± 0.025} & \textbf{0.846 ± 0.026} & \textbf{0.796 ± 0.010} & \underline{0.691 ± 0.058} & \textbf{0.928 ± 0.017} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.969 ± 0.003 & 0.836 ± 0.009 & \underline{0.867 ± 0.015} & 0.748 ± 0.034 & \underline{0.773 ± 0.044} & 0.588 ± 0.073 & \underline{0.884 ± 0.047} \\
& \prism\cite{} & \underline{0.978 ± 0.005} & \underline{0.859 ± 0.014} & 0.863 ± 0.017 & \underline{0.810 ± 0.013} & 0.704 ± 0.015 & \textbf{0.738 ± 0.032} & 0.877 ± 0.022 \\
& \gigapath\cite{} & 0.957 ± 0.003 & 0.838 ± 0.013 & 0.699 ± 0.022 & 0.653 ± 0.033 & 0.630 ± 0.040 & 0.485 ± 0.093 & 0.676 ± 0.067 \\
& $\ours$ & \textbf{0.982 ± 0.004} & \textbf{0.895 ± 0.011} & \textbf{0.898 ± 0.027} & \textbf{0.879 ± 0.020} & \textbf{0.817 ± 0.033} & \underline{0.725 ± 0.062} & \textbf{0.933 ± 0.026} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.980 ± 0.003 & 0.869 ± 0.014 & 0.855 ± 0.032 & 0.817 ± 0.034 & 0.817 ± 0.021 & \underline{0.666 ± 0.058} & \textbf{0.883 ± 0.035} \\
& \gigapath\cite{} & 0.986 ± 0.004 & \underline{0.890 ± 0.007} & 0.620 ± 0.050 & 0.682 ± 0.020 & 0.688 ± 0.029 & 0.496 ± 0.048 & 0.537 ± 0.102 \\
& $\ours$ Random Init & \underline{0.987 ± 0.002} & 0.889 ± 0.011 & \textbf{0.900 ± 0.022} & \underline{0.849 ± 0.026} & \textbf{0.824 ± 0.006} & 0.583 ± 0.070 & 0.867 ± 0.054 \\
& $\ours$ & \textbf{0.988 ± 0.001} & \textbf{0.892 ± 0.008} & \underline{0.893 ± 0.026} & \textbf{0.862 ± 0.022} & \underline{0.820 ± 0.017} & \textbf{0.724 ± 0.042} & \underline{0.874 ± 0.032} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mgb_lung}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on BCNB\cite{xu2021predicting} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{ER}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{PR}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{HER2}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & ER ($\uparrow$) (n=1057) & PR ($\uparrow$) (n=1057) & HER2 ($\uparrow$) (n=1057) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.833 ± 0.011 & 0.780 ± 0.024 & 0.692 ± 0.018 \\
& \prism\cite{} & \underline{0.843 ± 0.013} & \underline{0.792 ± 0.014} & \underline{0.734 ± 0.012} \\
& \gigapath\cite{} & 0.800 ± 0.017 & 0.755 ± 0.019 & 0.673 ± 0.021 \\
& $\ours$ & \textbf{0.896 ± 0.010} & \textbf{0.834 ± 0.017} & \textbf{0.753 ± 0.012} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.889 ± 0.010 & 0.810 ± 0.022 & \underline{0.737 ± 0.013} \\
& \prism\cite{} & \underline{0.892 ± 0.014} & \underline{0.816 ± 0.019} & 0.711 ± 0.010 \\
& \gigapath\cite{} & 0.886 ± 0.016 & 0.810 ± 0.013 & 0.701 ± 0.016 \\
& $\ours$ & \textbf{0.921 ± 0.009} & \textbf{0.837 ± 0.020} & \textbf{0.765 ± 0.008} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.880 ± 0.011 & 0.810 ± 0.011 & 0.736 ± 0.019 \\
& \gigapath\cite{} & \textbf{0.930 ± 0.009} & \textbf{0.858 ± 0.015} & 0.762 ± 0.018 \\
& $\ours$ Random Init & 0.920 ± 0.009 & \underline{0.855 ± 0.013} & \textbf{0.790 ± 0.008} \\
& $\ours$ & \underline{0.921 ± 0.013} & 0.840 ± 0.015 & \underline{0.788 ± 0.006} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_bcnb}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MUT-HET-RCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BAP1 Mutation}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{PBRM1 Mutation}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{SETD2 Mutation}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & BAP1 Mutation ($\uparrow$) (n=1291) & PBRM1 Mutation ($\uparrow$) (n=1291) & SETD2 Mutation ($\uparrow$) (n=1291) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.828 ± 0.022} & 0.673 ± 0.006 & \textbf{0.704 ± 0.009} \\
& \prism\cite{} & 0.827 ± 0.016 & \underline{0.701 ± 0.008} & 0.683 ± 0.015 \\
& \gigapath\cite{} & 0.823 ± 0.018 & 0.682 ± 0.004 & \underline{0.695 ± 0.015} \\
& $\ours$ & \textbf{0.851 ± 0.010} & \textbf{0.760 ± 0.003} & 0.689 ± 0.012 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.846 ± 0.011 & 0.781 ± 0.004 & 0.728 ± 0.011 \\
& \prism\cite{} & 0.848 ± 0.017 & \underline{0.798 ± 0.008} & \underline{0.733 ± 0.009} \\
& \gigapath\cite{} & \underline{0.858 ± 0.007} & 0.798 ± 0.003 & 0.712 ± 0.012 \\
& $\ours$ & \textbf{0.873 ± 0.006} & \textbf{0.826 ± 0.003} & \textbf{0.756 ± 0.009} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.884 ± 0.008 & 0.783 ± 0.009 & 0.717 ± 0.009 \\
& \gigapath\cite{} & \textbf{0.905 ± 0.004} & \textbf{0.820 ± 0.014} & 0.728 ± 0.009 \\
& $\ours$ Random Init & 0.880 ± 0.009 & 0.810 ± 0.006 & \underline{0.739 ± 0.005} \\
& $\ours$ & \underline{0.896 ± 0.007} & \underline{0.817 ± 0.008} & \textbf{0.741 ± 0.007} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mut-het-rcc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on IMP\cite{neto2024interpretable} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Grade}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Grade ($\uparrow$) (n=5333) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.791 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.929 ± TBD (0.000)} \\
& \gigapath\cite{} & \underline{0.839 ± TBD (0.000)} \\
& $\ours$ & 0.835 ± TBD (0.000) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.907 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.941 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.928 ± TBD (0.000) \\
& $\ours$ & \underline{0.933 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.949 ± TBD (0.000)} \\
& \gigapath\cite{} & \textbf{0.969 ± TBD (0.000)} \\
& $\ours$ Random Init & 0.947 ± TBD (0.000) \\
& $\ours$ & 0.946 ± TBD (0.000) \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_imp}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on PANDA\cite{bulten2022artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{ISUP Grade}: This is a slide-level classification task evaluated using quadratic weighted kappa, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & ISUP Grade ($\uparrow$) (n=9555) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.701 ± TBD (0.000) \\
& \prism\cite{} & \underline{0.809 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.465 ± TBD (0.000) \\
& $\ours$ & \textbf{0.814 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.844 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.919 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.872 ± TBD (0.000) \\
& $\ours$ & \underline{0.915 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.932 ± TBD (0.000) \\
& \gigapath\cite{} & \textbf{0.954 ± TBD (0.000)} \\
& $\ours$ Random Init & 0.930 ± TBD (0.000) \\
& $\ours$ & \underline{0.933 ± TBD (0.000)} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_panda}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-BRCA\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{PIK3CA Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & PIK3CA Mutation ($\uparrow$) (n=103) & TP53 Mutation ($\uparrow$) (n=103) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.602 ± 0.015} & 0.783 ± 0.014 \\
& \prism\cite{} & 0.578 ± 0.016 & \underline{0.839 ± 0.011} \\
& \gigapath\cite{} & 0.546 ± 0.018 & 0.743 ± 0.014 \\
& $\ours$ & \textbf{0.637 ± 0.014} & \textbf{0.873 ± 0.012} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.512 ± 0.017 & \underline{0.796 ± 0.011} \\
& \prism\cite{} & \textbf{0.575 ± 0.014} & 0.787 ± 0.013 \\
& \gigapath\cite{} & 0.536 ± 0.018 & 0.742 ± 0.013 \\
& $\ours$ & \underline{0.571 ± 0.017} & \textbf{0.876 ± 0.012} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.522 ± 0.015 & 0.791 ± 0.013 \\
& \gigapath\cite{} & 0.561 ± 0.016 & 0.768 ± 0.014 \\
& $\ours$ Random Init & \underline{0.579 ± 0.015} & \textbf{0.856 ± 0.012} \\
& $\ours$ & \textbf{0.605 ± 0.016} & \underline{0.846 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_brca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-CCRCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BAP1 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{PBRM1 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & BAP1 Mutation ($\uparrow$) (n=103) & PBRM1 Mutation ($\uparrow$) (n=103) & Survival ($\uparrow$) (n=94) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.723 ± 0.020 & 0.551 ± 0.018 & \textbf{} \\
& \prism\cite{} & \underline{0.729 ± 0.017} & \underline{0.593 ± 0.019} & \textbf{} \\
& \gigapath\cite{} & 0.679 ± 0.024 & 0.455 ± 0.016 & \textbf{} \\
& $\ours$ & \textbf{0.861 ± 0.009} & \textbf{0.635 ± 0.016} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.655 ± 0.016 & 0.518 ± 0.015 & \textbf{} \\
& \prism\cite{} & \underline{0.664 ± 0.022} & \underline{0.598 ± 0.019} & \textbf{} \\
& \gigapath\cite{} & 0.654 ± 0.024 & 0.497 ± 0.016 & \textbf{} \\
& $\ours$ & \textbf{0.809 ± 0.014} & \textbf{0.668 ± 0.016} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.724 ± 0.019 & 0.580 ± 0.019 & \textbf{} \\
& \gigapath\cite{} & 0.721 ± 0.019 & 0.484 ± 0.015 & \textbf{} \\
& $\ours$ Random Init & \textbf{0.788 ± 0.014} & \underline{0.603 ± 0.017} & \textbf{} \\
& $\ours$ & \underline{0.787 ± 0.016} & \textbf{0.631 ± 0.016} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_ccrcc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-COAD\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{KRAS Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & KRAS Mutation ($\uparrow$) (n=94) & TP53 Mutation ($\uparrow$) (n=94) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \textbf{0.655 ± 0.015} & \underline{0.657 ± 0.019} \\
& \prism\cite{} & 0.472 ± 0.016 & 0.581 ± 0.020 \\
& \gigapath\cite{} & 0.582 ± 0.015 & 0.633 ± 0.019 \\
& $\ours$ & \underline{0.621 ± 0.015} & \textbf{0.805 ± 0.014} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \textbf{0.742 ± 0.016} & \underline{0.690 ± 0.018} \\
& \prism\cite{} & 0.554 ± 0.015 & 0.578 ± 0.019 \\
& \gigapath\cite{} & 0.647 ± 0.014 & 0.648 ± 0.016 \\
& $\ours$ & \underline{0.704 ± 0.014} & \textbf{0.742 ± 0.016} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.628 ± 0.017 & \underline{0.747 ± 0.014} \\
& \gigapath\cite{} & 0.596 ± 0.014 & 0.635 ± 0.016 \\
& $\ours$ Random Init & \textbf{0.689 ± 0.015} & 0.715 ± 0.016 \\
& $\ours$ & \underline{0.665 ± 0.016} & \textbf{0.785 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_coad}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-GBM\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{EGFR Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & EGFR Mutation ($\uparrow$) (n=99) & TP53 Mutation ($\uparrow$) (n=99) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.654 ± 0.014} & 0.738 ± 0.017 \\
& \prism\cite{} & 0.586 ± 0.016 & \textbf{0.770 ± 0.017} \\
& \gigapath\cite{} & 0.618 ± 0.014 & 0.622 ± 0.019 \\
& $\ours$ & \textbf{0.757 ± 0.015} & \underline{0.744 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.639 ± 0.014} & 0.828 ± 0.014 \\
& \prism\cite{} & 0.618 ± 0.015 & \textbf{0.858 ± 0.015} \\
& \gigapath\cite{} & 0.633 ± 0.017 & 0.773 ± 0.014 \\
& $\ours$ & \textbf{0.782 ± 0.011} & \underline{0.842 ± 0.013} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.711 ± 0.015} & 0.835 ± 0.014 \\
& \gigapath\cite{} & 0.604 ± 0.015 & 0.643 ± 0.016 \\
& $\ours$ Random Init & 0.700 ± 0.012 & \underline{0.851 ± 0.013} \\
& $\ours$ & \textbf{0.791 ± 0.009} & \textbf{0.867 ± 0.012} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_gbm}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-HNSC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{CASP8 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & CASP8 Mutation ($\uparrow$) (n=107) & Survival ($\uparrow$) (n=102) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.675 ± 0.022} & \textbf{} \\
& \prism\cite{} & 0.674 ± 0.025 & \textbf{} \\
& \gigapath\cite{} & 0.602 ± 0.027 & \textbf{} \\
& $\ours$ & \textbf{0.778 ± 0.018} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.614 ± 0.028} & \textbf{} \\
& \prism\cite{} & 0.601 ± 0.027 & \textbf{} \\
& \gigapath\cite{} & 0.501 ± 0.023 & \textbf{} \\
& $\ours$ & \textbf{0.754 ± 0.019} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.657 ± 0.033 & \textbf{} \\
& \gigapath\cite{} & 0.614 ± 0.027 & \textbf{} \\
& $\ours$ Random Init & \underline{0.695 ± 0.022} & \textbf{} \\
& $\ours$ & \textbf{0.733 ± 0.025} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_hnsc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-LSCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{KEAP1 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{ARID1A Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & KEAP1 Mutation ($\uparrow$) (n=108) & ARID1A Mutation ($\uparrow$) (n=108) & Survival ($\uparrow$) (n=94) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \textbf{0.669 ± 0.017} & 0.521 ± 0.020 & \textbf{} \\
& \prism\cite{} & 0.456 ± 0.018 & 0.548 ± 0.023 & \textbf{} \\
& \gigapath\cite{} & 0.576 ± 0.021 & \underline{0.590 ± 0.020} & \textbf{} \\
& $\ours$ & \underline{0.646 ± 0.021} & \textbf{0.610 ± 0.027} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.574 ± 0.018 & 0.411 ± 0.020 & \textbf{} \\
& \prism\cite{} & 0.491 ± 0.018 & 0.449 ± 0.020 & \textbf{} \\
& \gigapath\cite{} & \underline{0.644 ± 0.018} & \underline{0.490 ± 0.017} & \textbf{} \\
& $\ours$ & \textbf{0.685 ± 0.019} & \textbf{0.658 ± 0.023} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.470 ± 0.023 & 0.469 ± 0.027 & \textbf{} \\
& \gigapath\cite{} & \underline{0.613 ± 0.020} & \textbf{0.553 ± 0.019} & \textbf{} \\
& $\ours$ Random Init & 0.601 ± 0.019 & 0.466 ± 0.018 & \textbf{} \\
& $\ours$ & \textbf{0.614 ± 0.017} & \underline{0.508 ± 0.023} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_lscc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-LUAD\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{EGFR Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{STK11 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{4}{c}{Tasks} \\ 
\cmidrule(lr){3-6}
& & EGFR Mutation ($\uparrow$) (n=108) & STK11 Mutation ($\uparrow$) (n=108) & TP53 Mutation ($\uparrow$) (n=108) & Survival ($\uparrow$) (n=105) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.748 ± 0.017} & 0.810 ± 0.020 & 0.663 ± 0.016 & \textbf{} \\
& \prism\cite{} & 0.722 ± 0.016 & \underline{0.875 ± 0.015} & \underline{0.688 ± 0.016} & \textbf{} \\
& \gigapath\cite{} & 0.723 ± 0.018 & 0.770 ± 0.022 & 0.631 ± 0.018 & \textbf{} \\
& $\ours$ & \textbf{0.767 ± 0.014} & \textbf{0.893 ± 0.015} & \textbf{0.722 ± 0.014} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.789 ± 0.014 & 0.824 ± 0.018 & 0.682 ± 0.015 & \textbf{} \\
& \prism\cite{} & \underline{0.809 ± 0.013} & \underline{0.854 ± 0.015} & \textbf{0.756 ± 0.013} & \textbf{} \\
& \gigapath\cite{} & 0.786 ± 0.014 & 0.827 ± 0.014 & 0.733 ± 0.013 & \textbf{} \\
& $\ours$ & \textbf{0.822 ± 0.011} & \textbf{0.889 ± 0.015} & \underline{0.752 ± 0.014} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.761 ± 0.016 & 0.840 ± 0.015 & 0.671 ± 0.015 & \textbf{} \\
& \gigapath\cite{} & 0.732 ± 0.015 & 0.812 ± 0.017 & 0.695 ± 0.017 & \textbf{} \\
& $\ours$ Random Init & \textbf{0.809 ± 0.014} & \underline{0.869 ± 0.015} & \underline{0.719 ± 0.015} & \textbf{} \\
& $\ours$ & \underline{0.792 ± 0.015} & \textbf{0.895 ± 0.011} & \textbf{0.758 ± 0.013} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_luad}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-PDAC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{SMAD4 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & SMAD4 Mutation ($\uparrow$) (n=105) & Survival ($\uparrow$) (n=97) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.606 ± 0.021} & \textbf{} \\
& \prism\cite{} & 0.593 ± 0.023 & \textbf{} \\
& \gigapath\cite{} & 0.311 ± 0.020 & \textbf{} \\
& $\ours$ & \textbf{0.666 ± 0.022} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.576 ± 0.020} & \textbf{} \\
& \prism\cite{} & 0.523 ± 0.022 & \textbf{} \\
& \gigapath\cite{} & 0.426 ± 0.021 & \textbf{} \\
& $\ours$ & \textbf{0.578 ± 0.024} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.502 ± 0.019 & \textbf{} \\
& \gigapath\cite{} & 0.331 ± 0.018 & \textbf{} \\
& $\ours$ Random Init & \textbf{0.598 ± 0.021} & \textbf{} \\
& $\ours$ & \underline{0.582 ± 0.022} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_pda}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on BRACS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Fine Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and standard error reported over 5-fold cross-validation. \textbf{Coarse Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=547) & Coarse Subtype ($\uparrow$) (n=547) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.336 ± 0.019 & 0.645 ± 0.020 \\
& \prism\cite{} & \textbf{0.474 ± 0.027} & \textbf{0.726 ± 0.020} \\
& \gigapath\cite{} & 0.286 ± 0.018 & 0.575 ± 0.033 \\
& $\ours$ & \underline{0.452 ± 0.024} & \underline{0.724 ± 0.028} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.377 ± 0.036 & 0.623 ± 0.036 \\
& \prism\cite{} & \underline{0.420 ± 0.015} & \underline{0.658 ± 0.019} \\
& \gigapath\cite{} & 0.339 ± 0.018 & 0.608 ± 0.034 \\
& $\ours$ & \textbf{0.481 ± 0.015} & \textbf{0.716 ± 0.019} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \textbf{0.504 ± 0.010} & 0.696 ± 0.031 \\
& \gigapath\cite{} & 0.459 ± 0.020 & 0.681 ± 0.020 \\
& $\ours$ Random Init & \underline{0.485 ± 0.019} & \textbf{0.757 ± 0.019} \\
& $\ours$ & 0.479 ± 0.022 & \underline{0.725 ± 0.019} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_bracs}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on eBRAINS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Fine Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. \textbf{Coarse Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=2319) & Coarse Subtype ($\uparrow$) (n=2319) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.549 ± TBD (0.000) & 0.724 ± TBD (0.000) \\
& \prism\cite{} & \underline{0.624 ± TBD (0.000)} & \underline{0.752 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.617 ± TBD (0.000) & 0.745 ± TBD (0.000) \\
& $\ours$ & \textbf{0.705 ± TBD (0.000)} & \textbf{0.839 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.693 ± TBD (0.000) & 0.874 ± TBD (0.000) \\
& \prism\cite{} & 0.714 ± TBD (0.000) & 0.872 ± TBD (0.000) \\
& \gigapath\cite{} & \underline{0.722 ± TBD (0.000)} & \underline{0.892 ± TBD (0.000)} \\
& $\ours$ & \textbf{0.741 ± TBD (0.000)} & \textbf{0.919 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.722 ± TBD (0.000) & 0.882 ± TBD (0.000) \\
& \gigapath\cite{} & \textbf{0.747 ± TBD (0.000)} & \textbf{0.905 ± TBD (0.000)} \\
& $\ours$ Random Init & \textbf{0.747 ± TBD (0.000)} & \textbf{0.905 ± TBD (0.000)} \\
& $\ours$ & 0.741 ± TBD (0.000) & 0.895 ± TBD (0.000) \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_ebrains}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on IMPRESS-HER2\cite{huang2023artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{pCR}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & pCR ($\uparrow$) (n=62) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.474 ± 0.020 \\
& \prism\cite{} & \textbf{0.667 ± 0.022} \\
& \gigapath\cite{} & 0.601 ± 0.019 \\
& $\ours$ & \underline{0.611 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.472 ± 0.019 \\
& \prism\cite{} & \textbf{0.642 ± 0.019} \\
& \gigapath\cite{} & 0.565 ± 0.022 \\
& $\ours$ & \underline{0.603 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.701 ± 0.022} \\
& \gigapath\cite{} & 0.533 ± 0.018 \\
& $\ours$ Random Init & 0.531 ± 0.019 \\
& $\ours$ & \textbf{0.709 ± 0.019} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_impress_her2}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on IMPRESS-TNBC\cite{huang2023artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{pCR}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & pCR ($\uparrow$) (n=64) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.570 ± 0.022 \\
& \prism\cite{} & 0.587 ± 0.021 \\
& \gigapath\cite{} & \underline{0.598 ± 0.020} \\
& $\ours$ & \textbf{0.657 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \textbf{0.652 ± 0.020} \\
& \prism\cite{} & 0.541 ± 0.017 \\
& \gigapath\cite{} & \underline{0.617 ± 0.018} \\
& $\ours$ & 0.602 ± 0.021 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.615 ± 0.020} \\
& \gigapath\cite{} & 0.595 ± 0.021 \\
& $\ours$ Random Init & \textbf{0.644 ± 0.020} \\
& $\ours$ & 0.604 ± 0.022 \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_impress_tnbc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on OV-Bevacizumab\cite{wang2022weakly} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Response}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=36) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.797 ± 0.026} \\
& \prism\cite{} & 0.443 ± 0.041 \\
& \gigapath\cite{} & 0.760 ± 0.028 \\
& $\ours$ & \textbf{0.857 ± 0.025} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.623 ± 0.030} \\
& \prism\cite{} & 0.433 ± 0.034 \\
& \gigapath\cite{} & 0.603 ± 0.039 \\
& $\ours$ & \textbf{0.863 ± 0.021} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.540 ± 0.033 \\
& \gigapath\cite{} & 0.457 ± 0.046 \\
& $\ours$ Random Init & \underline{0.753 ± 0.028} \\
& $\ours$ & \textbf{0.780 ± 0.032} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_ovarian}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on NADT Prostate\cite{wilkinson2021nascent} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Response}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=36) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.683 ± 0.022 \\
& \prism\cite{} & \textbf{0.752 ± 0.024} \\
& \gigapath\cite{} & 0.688 ± 0.026 \\
& $\ours$ & \underline{0.725 ± 0.023} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.622 ± 0.026 \\
& \prism\cite{} & \underline{0.720 ± 0.023} \\
& \gigapath\cite{} & 0.577 ± 0.024 \\
& $\ours$ & \textbf{0.730 ± 0.022} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.583 ± 0.033 \\
& \gigapath\cite{} & 0.525 ± 0.036 \\
& $\ours$ Random Init & \textbf{0.717 ± 0.022} \\
& $\ours$ & \underline{0.702 ± 0.020} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_nadt}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on GBM-Treatment\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Response}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=93) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.668 ± 0.018} \\
& \prism\cite{} & 0.633 ± 0.019 \\
& \gigapath\cite{} & \textbf{0.672 ± 0.016} \\
& $\ours$ & 0.659 ± 0.018 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.703 ± 0.018} \\
& \prism\cite{} & 0.622 ± 0.022 \\
& \gigapath\cite{} & 0.618 ± 0.017 \\
& $\ours$ & \textbf{0.741 ± 0.016} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.704 ± 0.018} \\
& \gigapath\cite{} & 0.642 ± 0.017 \\
& $\ours$ Random Init & 0.660 ± 0.018 \\
& $\ours$ & \textbf{0.707 ± 0.016} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_gbm_rt_tmz}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on Post-NAT-BRCA\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Lymphovascular Invasion}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Lymphovascular Invasion ($\uparrow$) (n=53) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & 0.568 ± 0.026 \\
& \prism\cite{} & 0.487 ± 0.024 \\
& \gigapath\cite{} & \textbf{0.627 ± 0.025} \\
& $\ours$ & \underline{0.601 ± 0.027} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & \underline{0.654 ± 0.022} \\
& \prism\cite{} & 0.540 ± 0.029 \\
& \gigapath\cite{} & 0.577 ± 0.024 \\
& $\ours$ & \textbf{0.701 ± 0.027} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.553 ± 0.025 \\
& \gigapath\cite{} & \underline{0.615 ± 0.025} \\
& $\ours$ Random Init & 0.580 ± 0.023 \\
& $\ours$ & \textbf{0.662 ± 0.028} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_natbrca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on SURGEN\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BRAF Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{RAS Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{MMR Loss}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Death in 5 Years}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Survival}: This is a patient-level survival task evaluated using C-index, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{5}{c}{Tasks} \\ 
\cmidrule(lr){3-7}
& & BRAF Mutation ($\uparrow$) (n=388) & RAS Mutation ($\uparrow$) (n=389) & MMR Loss ($\uparrow$) (n=389) & Death in 5 Years ($\uparrow$) (n=387) & Survival ($\uparrow$) (n=144) \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \mean & \underline{0.641 ± 0.020} & \underline{0.619 ± 0.020} & \underline{0.819 ± 0.026} & \underline{0.663 ± 0.023} & \textbf{} \\
& \prism\cite{} &  &  &  &  & \textbf{} \\
& \gigapath\cite{} & 0.616 ± 0.021 & 0.618 ± 0.010 & 0.779 ± 0.046 & 0.631 ± 0.024 & \textbf{} \\
& $\ours$ & \textbf{0.753 ± 0.039} & \textbf{0.649 ± 0.029} & \textbf{0.914 ± 0.019} & \textbf{0.667 ± 0.017} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \mean & 0.649 ± 0.025 & \underline{0.630 ± 0.028} & 0.797 ± 0.037 & \underline{0.661 ± 0.023} & \textbf{} \\
& \prism\cite{} &  &  &  &  & \textbf{} \\
& \gigapath\cite{} & \underline{0.679 ± 0.026} & 0.621 ± 0.022 & \underline{0.861 ± 0.015} & 0.633 ± 0.013 & \textbf{} \\
& $\ours$ & \textbf{0.726 ± 0.042} & \textbf{0.632 ± 0.027} & \textbf{0.910 ± 0.023} & \textbf{0.685 ± 0.017} & \textbf{} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.692 ± 0.046 & \underline{0.656 ± 0.017} & 0.841 ± 0.035 & 0.695 ± 0.017 & \textbf{} \\
& \gigapath\cite{} &  &  &  &  & \textbf{} \\
& $\ours$ Random Init & \underline{0.715 ± 0.032} & 0.635 ± 0.026 & \underline{0.893 ± 0.030} & \underline{0.703 ± 0.029} & \textbf{} \\
& $\ours$ & \textbf{0.798 ± 0.031} & \textbf{0.675 ± 0.014} & \textbf{0.894 ± 0.035} & \textbf{0.733 ± 0.024} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_sr386_}
\end{table}




==> tables/archived/downstream_performance_withmeans.tex <==
\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MGB Breast tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Subtype}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{ER}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{PR}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{HER2}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{4}{c}{Tasks} \\ 
\cmidrule(lr){3-6}
& & Subtype ($\uparrow$) (n=1264) & ER ($\uparrow$) (n=874) & PR ($\uparrow$) (n=874) & HER2 ($\uparrow$) (n=816) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.763 ± 0.014 & 0.640 ± 0.024 & 0.632 ± 0.013 & 0.535 ± 0.034 \\
& \prism\cite{} & \textbf{0.982 ± 0.003} & \underline{0.780 ± 0.020} & \underline{0.738 ± 0.020} & \textbf{0.708 ± 0.026} \\
& \gigapath\cite{} \mean & 0.864 ± 0.013 & 0.708 ± 0.017 & 0.695 ± 0.013 & 0.588 ± 0.028 \\
& \gigapath\cite{} & 0.842 ± 0.014 & 0.694 ± 0.018 & 0.687 ± 0.015 & 0.567 ± 0.030 \\
& \mean & 0.868 ± 0.013 & 0.691 ± 0.012 & 0.670 ± 0.015 & 0.588 ± 0.029 \\
& $\ours$ & \underline{0.922 ± 0.006} & \textbf{0.784 ± 0.017} & \textbf{0.741 ± 0.019} & \underline{0.701 ± 0.027} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.971 ± 0.003 & 0.705 ± 0.016 & 0.672 ± 0.012 & 0.599 ± 0.020 \\
& \prism\cite{} & \textbf{0.985 ± 0.002} & 0.727 ± 0.022 & 0.639 ± 0.001 & \textbf{0.710 ± 0.021} \\
& \gigapath\cite{} \mean & 0.979 ± 0.002 & 0.711 ± 0.012 & 0.682 ± 0.018 & 0.575 ± 0.014 \\
& \gigapath\cite{} & 0.974 ± 0.003 & 0.709 ± 0.014 & 0.689 ± 0.020 & 0.596 ± 0.010 \\
& \conch\cite{} \mean & 0.973 ± 0.005 & \underline{0.728 ± 0.026} & \underline{0.720 ± 0.012} & 0.656 ± 0.042 \\
& $\ours$ & \underline{0.983 ± 0.004} & \textbf{0.784 ± 0.016} & \textbf{0.748 ± 0.021} & \underline{0.694 ± 0.031} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.983 ± 0.004 & 0.720 ± 0.025 & 0.690 ± 0.007 & 0.622 ± 0.012 \\
& \gigapath\cite{} & \textbf{0.988 ± 0.001} & 0.756 ± 0.017 & 0.728 ± 0.015 & 0.682 ± 0.021 \\
& $\ours$ Random Init & \underline{0.985 ± 0.003} & \textbf{0.780 ± 0.024} & \textbf{0.757 ± 0.016} & \textbf{0.701 ± 0.040} \\
& $\ours$ & 0.985 ± 0.003 & \underline{0.774 ± 0.026} & \underline{0.745 ± 0.019} & \underline{0.693 ± 0.037} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mgb_brca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MGB Lung tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Subtype}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{TTF-1}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{P40}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{P63}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Napsina}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{CDX-2}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{CK5-6}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccccccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{7}{c}{Tasks} \\ 
\cmidrule(lr){3-9}
& & Subtype ($\uparrow$) (n=1939) & TTF-1 ($\uparrow$) (n=488) & P40 ($\uparrow$) (n=185) & P63 ($\uparrow$) (n=153) & Napsina ($\uparrow$) (n=126) & CDX-2 ($\uparrow$) (n=79) & CK5-6 ($\uparrow$) (n=58) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.728 ± 0.006 & 0.621 ± 0.032 & 0.416 ± 0.027 & 0.633 ± 0.061 & 0.607 ± 0.047 & 0.490 ± 0.042 & 0.663 ± 0.090 \\
& \prism\cite{} & \textbf{0.988 ± 0.002} & \textbf{0.890 ± 0.012} & \underline{0.885 ± 0.029} & \underline{0.793 ± 0.052} & \underline{0.786 ± 0.021} & \textbf{0.720 ± 0.061} & \underline{0.890 ± 0.026} \\
& \gigapath\cite{} \mean & 0.785 ± 0.006 & 0.658 ± 0.025 & 0.465 ± 0.015 & 0.638 ± 0.039 & 0.622 ± 0.033 & 0.505 ± 0.069 & 0.639 ± 0.083 \\
& \gigapath\cite{} & 0.754 ± 0.007 & 0.629 ± 0.022 & 0.401 ± 0.007 & 0.633 ± 0.036 & 0.605 ± 0.029 & 0.452 ± 0.047 & 0.661 ± 0.090 \\
& \mean & 0.830 ± 0.007 & 0.699 ± 0.027 & 0.637 ± 0.021 & 0.681 ± 0.052 & 0.669 ± 0.037 & 0.628 ± 0.081 & 0.748 ± 0.072 \\
& $\ours$ & \underline{0.983 ± 0.002} & \underline{0.864 ± 0.020} & \textbf{0.897 ± 0.025} & \textbf{0.846 ± 0.026} & \textbf{0.796 ± 0.010} & \underline{0.691 ± 0.058} & \textbf{0.928 ± 0.017} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.960 ± 0.002 & 0.837 ± 0.017 & 0.750 ± 0.033 & 0.640 ± 0.036 & 0.678 ± 0.050 & 0.529 ± 0.050 & 0.742 ± 0.051 \\
& \prism\cite{} & \underline{0.978 ± 0.005} & 0.859 ± 0.014 & 0.863 ± 0.017 & \underline{0.810 ± 0.013} & 0.704 ± 0.015 & \textbf{0.738 ± 0.032} & 0.877 ± 0.022 \\
& \gigapath\cite{} \mean & 0.969 ± 0.002 & \underline{0.866 ± 0.008} & 0.739 ± 0.019 & 0.681 ± 0.027 & 0.693 ± 0.031 & 0.506 ± 0.092 & 0.697 ± 0.050 \\
& \gigapath\cite{} & 0.957 ± 0.003 & 0.838 ± 0.013 & 0.699 ± 0.022 & 0.653 ± 0.033 & 0.630 ± 0.040 & 0.485 ± 0.093 & 0.676 ± 0.067 \\
& \conch\cite{} \mean & 0.969 ± 0.003 & 0.836 ± 0.009 & \underline{0.867 ± 0.015} & 0.748 ± 0.034 & \underline{0.773 ± 0.044} & 0.588 ± 0.073 & \underline{0.884 ± 0.047} \\
& $\ours$ & \textbf{0.982 ± 0.004} & \textbf{0.895 ± 0.011} & \textbf{0.898 ± 0.027} & \textbf{0.879 ± 0.020} & \textbf{0.817 ± 0.033} & \underline{0.725 ± 0.062} & \textbf{0.933 ± 0.026} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.980 ± 0.003 & 0.869 ± 0.014 & 0.855 ± 0.032 & 0.817 ± 0.034 & 0.817 ± 0.021 & \underline{0.666 ± 0.058} & \textbf{0.883 ± 0.035} \\
& \gigapath\cite{} & 0.986 ± 0.004 & \underline{0.890 ± 0.007} & 0.620 ± 0.050 & 0.682 ± 0.020 & 0.688 ± 0.029 & 0.496 ± 0.048 & 0.537 ± 0.102 \\
& $\ours$ Random Init & \underline{0.987 ± 0.002} & 0.889 ± 0.011 & \textbf{0.900 ± 0.022} & \underline{0.849 ± 0.026} & \textbf{0.824 ± 0.006} & 0.583 ± 0.070 & 0.867 ± 0.054 \\
& $\ours$ & \textbf{0.988 ± 0.001} & \textbf{0.892 ± 0.008} & \underline{0.893 ± 0.026} & \textbf{0.862 ± 0.022} & \underline{0.820 ± 0.017} & \textbf{0.724 ± 0.042} & \underline{0.874 ± 0.032} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mgb_lung}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on BCNB\cite{xu2021predicting} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{ER}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{PR}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{HER2}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & ER ($\uparrow$) (n=1057) & PR ($\uparrow$) (n=1057) & HER2 ($\uparrow$) (n=1057) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.713 ± 0.029 & 0.681 ± 0.033 & 0.630 ± 0.018 \\
& \prism\cite{} & \underline{0.843 ± 0.013} & \underline{0.792 ± 0.014} & \underline{0.734 ± 0.012} \\
& \gigapath\cite{} \mean & 0.811 ± 0.015 & 0.763 ± 0.019 & 0.679 ± 0.022 \\
& \gigapath\cite{} & 0.800 ± 0.017 & 0.755 ± 0.019 & 0.673 ± 0.021 \\
& \mean & 0.833 ± 0.011 & 0.780 ± 0.024 & 0.692 ± 0.018 \\
& $\ours$ & \textbf{0.896 ± 0.010} & \textbf{0.834 ± 0.017} & \textbf{0.753 ± 0.012} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.888 ± 0.007 & 0.813 ± 0.010 & 0.707 ± 0.011 \\
& \prism\cite{} & 0.892 ± 0.014 & 0.816 ± 0.019 & 0.711 ± 0.010 \\
& \gigapath\cite{} \mean & \underline{0.901 ± 0.013} & \underline{0.828 ± 0.013} & 0.718 ± 0.015 \\
& \gigapath\cite{} & 0.886 ± 0.016 & 0.810 ± 0.013 & 0.701 ± 0.016 \\
& \conch\cite{} \mean & 0.889 ± 0.010 & 0.810 ± 0.022 & \underline{0.737 ± 0.013} \\
& $\ours$ & \textbf{0.921 ± 0.009} & \textbf{0.837 ± 0.020} & \textbf{0.765 ± 0.008} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.880 ± 0.011 & 0.810 ± 0.011 & 0.736 ± 0.019 \\
& \gigapath\cite{} & \textbf{0.930 ± 0.009} & \textbf{0.858 ± 0.015} & 0.762 ± 0.018 \\
& $\ours$ Random Init & 0.920 ± 0.009 & \underline{0.855 ± 0.013} & \textbf{0.790 ± 0.008} \\
& $\ours$ & \underline{0.921 ± 0.013} & 0.840 ± 0.015 & \underline{0.788 ± 0.006} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_bcnb}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MUT-HET-RCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BAP1 Mutation}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{PBRM1 Mutation}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{SETD2 Mutation}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & BAP1 Mutation ($\uparrow$) (n=1291) & PBRM1 Mutation ($\uparrow$) (n=1291) & SETD2 Mutation ($\uparrow$) (n=1291) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.811 ± 0.019 & 0.681 ± 0.004 & 0.682 ± 0.015 \\
& \prism\cite{} & 0.827 ± 0.016 & \underline{0.701 ± 0.008} & 0.683 ± 0.015 \\
& \gigapath\cite{} \mean & 0.812 ± 0.020 & 0.673 ± 0.005 & 0.684 ± 0.015 \\
& \gigapath\cite{} & 0.823 ± 0.018 & 0.682 ± 0.004 & \underline{0.695 ± 0.015} \\
& \mean & \underline{0.828 ± 0.022} & 0.673 ± 0.006 & \textbf{0.704 ± 0.009} \\
& $\ours$ & \textbf{0.851 ± 0.010} & \textbf{0.760 ± 0.003} & 0.689 ± 0.012 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & \underline{0.879 ± 0.003} & \underline{0.810 ± 0.008} & 0.712 ± 0.012 \\
& \prism\cite{} & 0.848 ± 0.017 & 0.798 ± 0.008 & \underline{0.733 ± 0.009} \\
& \gigapath\cite{} \mean & \textbf{0.880 ± 0.007} & 0.806 ± 0.007 & 0.701 ± 0.012 \\
& \gigapath\cite{} & 0.858 ± 0.007 & 0.798 ± 0.003 & 0.712 ± 0.012 \\
& \conch\cite{} \mean & 0.846 ± 0.011 & 0.781 ± 0.004 & 0.728 ± 0.011 \\
& $\ours$ & 0.873 ± 0.006 & \textbf{0.826 ± 0.003} & \textbf{0.756 ± 0.009} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.884 ± 0.008 & 0.783 ± 0.009 & 0.717 ± 0.009 \\
& \gigapath\cite{} & \textbf{0.905 ± 0.004} & \textbf{0.820 ± 0.014} & 0.728 ± 0.009 \\
& $\ours$ Random Init & 0.880 ± 0.009 & 0.810 ± 0.006 & \underline{0.739 ± 0.005} \\
& $\ours$ & \underline{0.896 ± 0.007} & \underline{0.817 ± 0.008} & \textbf{0.741 ± 0.007} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mut-het-rcc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on IMP\cite{neto2024interpretable} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Grade}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Grade ($\uparrow$) (n=5333) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.830 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.929 ± TBD (0.000)} \\
& \gigapath\cite{} \mean & \underline{0.848 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.839 ± TBD (0.000) \\
& \mean & 0.791 ± TBD (0.000) \\
& $\ours$ & 0.835 ± TBD (0.000) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.924 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.941 ± TBD (0.000)} \\
& \gigapath\cite{} \mean & 0.923 ± TBD (0.000) \\
& \gigapath\cite{} & 0.928 ± TBD (0.000) \\
& \conch\cite{} \mean & 0.907 ± TBD (0.000) \\
& $\ours$ & \underline{0.933 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.949 ± TBD (0.000)} \\
& \gigapath\cite{} & \textbf{0.969 ± TBD (0.000)} \\
& $\ours$ Random Init & 0.947 ± TBD (0.000) \\
& $\ours$ & 0.946 ± TBD (0.000) \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_imp}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on PANDA\cite{bulten2022artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{ISUP Grade}: This is a slide-level classification task evaluated using quadratic weighted kappa, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & ISUP Grade ($\uparrow$) (n=9555) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.467 ± TBD (0.000) \\
& \prism\cite{} & \underline{0.809 ± TBD (0.000)} \\
& \gigapath\cite{} \mean & 0.484 ± TBD (0.000) \\
& \gigapath\cite{} & 0.465 ± TBD (0.000) \\
& \mean & 0.701 ± TBD (0.000) \\
& $\ours$ & \textbf{0.814 ± TBD (0.000)} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.894 ± TBD (0.000) \\
& \prism\cite{} & \textbf{0.919 ± TBD (0.000)} \\
& \gigapath\cite{} \mean & 0.894 ± TBD (0.000) \\
& \gigapath\cite{} & 0.872 ± TBD (0.000) \\
& \conch\cite{} \mean & 0.844 ± TBD (0.000) \\
& $\ours$ & \underline{0.915 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.932 ± TBD (0.000) \\
& \gigapath\cite{} & \textbf{0.954 ± TBD (0.000)} \\
& $\ours$ Random Init & 0.930 ± TBD (0.000) \\
& $\ours$ & \underline{0.933 ± TBD (0.000)} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_panda}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-BRCA\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{PIK3CA Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & PIK3CA Mutation ($\uparrow$) (n=103) & TP53 Mutation ($\uparrow$) (n=103) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.594 ± 0.014 & 0.670 ± 0.015 \\
& \prism\cite{} & 0.578 ± 0.016 & \underline{0.839 ± 0.011} \\
& \gigapath\cite{} \mean & 0.589 ± 0.016 & 0.767 ± 0.014 \\
& \gigapath\cite{} & 0.546 ± 0.018 & 0.743 ± 0.014 \\
& \mean & \underline{0.602 ± 0.015} & 0.783 ± 0.014 \\
& $\ours$ & \textbf{0.637 ± 0.014} & \textbf{0.873 ± 0.012} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.569 ± 0.015 & 0.766 ± 0.012 \\
& \prism\cite{} & \textbf{0.575 ± 0.014} & 0.787 ± 0.013 \\
& \gigapath\cite{} \mean & 0.554 ± 0.016 & 0.754 ± 0.012 \\
& \gigapath\cite{} & 0.536 ± 0.018 & 0.742 ± 0.013 \\
& \conch\cite{} \mean & 0.512 ± 0.017 & \underline{0.796 ± 0.011} \\
& $\ours$ & \underline{0.571 ± 0.017} & \textbf{0.876 ± 0.012} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.522 ± 0.015 & 0.791 ± 0.013 \\
& \gigapath\cite{} & 0.561 ± 0.016 & 0.768 ± 0.014 \\
& $\ours$ Random Init & \underline{0.579 ± 0.015} & \textbf{0.856 ± 0.012} \\
& $\ours$ & \textbf{0.605 ± 0.016} & \underline{0.846 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_brca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-CCRCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BAP1 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{PBRM1 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & BAP1 Mutation ($\uparrow$) (n=103) & PBRM1 Mutation ($\uparrow$) (n=103) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & \underline{0.738 ± 0.020} & 0.446 ± 0.016 \\
& \prism\cite{} & 0.729 ± 0.017 & \underline{0.593 ± 0.019} \\
& \gigapath\cite{} \mean & 0.703 ± 0.023 & 0.434 ± 0.015 \\
& \gigapath\cite{} & 0.679 ± 0.024 & 0.455 ± 0.016 \\
& \mean & 0.723 ± 0.020 & 0.551 ± 0.018 \\
& $\ours$ & \textbf{0.861 ± 0.009} & \textbf{0.635 ± 0.016} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.624 ± 0.022 & 0.502 ± 0.016 \\
& \prism\cite{} & 0.664 ± 0.022 & \underline{0.598 ± 0.019} \\
& \gigapath\cite{} \mean & \underline{0.688 ± 0.023} & 0.482 ± 0.015 \\
& \gigapath\cite{} & 0.654 ± 0.024 & 0.497 ± 0.016 \\
& \conch\cite{} \mean & 0.655 ± 0.016 & 0.518 ± 0.015 \\
& $\ours$ & \textbf{0.809 ± 0.014} & \textbf{0.668 ± 0.016} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.724 ± 0.019 & 0.580 ± 0.019 \\
& \gigapath\cite{} & 0.721 ± 0.019 & 0.484 ± 0.015 \\
& $\ours$ Random Init & \textbf{0.788 ± 0.014} & \underline{0.603 ± 0.017} \\
& $\ours$ & \underline{0.787 ± 0.016} & \textbf{0.631 ± 0.016} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_ccrcc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-COAD\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{KRAS Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & KRAS Mutation ($\uparrow$) (n=94) & TP53 Mutation ($\uparrow$) (n=94) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.515 ± 0.018 & 0.595 ± 0.019 \\
& \prism\cite{} & 0.472 ± 0.016 & 0.581 ± 0.020 \\
& \gigapath\cite{} \mean & 0.597 ± 0.016 & 0.648 ± 0.017 \\
& \gigapath\cite{} & 0.582 ± 0.015 & 0.633 ± 0.019 \\
& \mean & \textbf{0.655 ± 0.015} & \underline{0.657 ± 0.019} \\
& $\ours$ & \underline{0.621 ± 0.015} & \textbf{0.805 ± 0.014} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.661 ± 0.015 & 0.684 ± 0.017 \\
& \prism\cite{} & 0.554 ± 0.015 & 0.578 ± 0.019 \\
& \gigapath\cite{} \mean & 0.642 ± 0.015 & 0.656 ± 0.018 \\
& \gigapath\cite{} & 0.647 ± 0.014 & 0.648 ± 0.016 \\
& \conch\cite{} \mean & \textbf{0.742 ± 0.016} & \underline{0.690 ± 0.018} \\
& $\ours$ & \underline{0.704 ± 0.014} & \textbf{0.742 ± 0.016} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.628 ± 0.017 & \underline{0.747 ± 0.014} \\
& \gigapath\cite{} & 0.596 ± 0.014 & 0.635 ± 0.016 \\
& $\ours$ Random Init & \textbf{0.689 ± 0.015} & 0.715 ± 0.016 \\
& $\ours$ & \underline{0.665 ± 0.016} & \textbf{0.785 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_coad}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-GBM\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{EGFR Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & EGFR Mutation ($\uparrow$) (n=99) & TP53 Mutation ($\uparrow$) (n=99) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.653 ± 0.013 & 0.597 ± 0.014 \\
& \prism\cite{} & 0.586 ± 0.016 & \textbf{0.770 ± 0.017} \\
& \gigapath\cite{} \mean & 0.627 ± 0.015 & 0.613 ± 0.021 \\
& \gigapath\cite{} & 0.618 ± 0.014 & 0.622 ± 0.019 \\
& \mean & \underline{0.654 ± 0.014} & 0.738 ± 0.017 \\
& $\ours$ & \textbf{0.757 ± 0.015} & \underline{0.744 ± 0.020} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.509 ± 0.017 & 0.816 ± 0.012 \\
& \prism\cite{} & 0.618 ± 0.015 & \textbf{0.858 ± 0.015} \\
& \gigapath\cite{} \mean & 0.623 ± 0.016 & 0.805 ± 0.012 \\
& \gigapath\cite{} & 0.633 ± 0.017 & 0.773 ± 0.014 \\
& \conch\cite{} \mean & \underline{0.639 ± 0.014} & 0.828 ± 0.014 \\
& $\ours$ & \textbf{0.782 ± 0.011} & \underline{0.842 ± 0.013} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.711 ± 0.015} & 0.835 ± 0.014 \\
& \gigapath\cite{} & 0.604 ± 0.015 & 0.643 ± 0.016 \\
& $\ours$ Random Init & 0.700 ± 0.012 & \underline{0.851 ± 0.013} \\
& $\ours$ & \textbf{0.791 ± 0.009} & \textbf{0.867 ± 0.012} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_gbm}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-HNSC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{CASP8 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & CASP8 Mutation ($\uparrow$) (n=107) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.626 ± 0.023 \\
& \prism\cite{} & 0.674 ± 0.025 \\
& \gigapath\cite{} \mean & 0.607 ± 0.030 \\
& \gigapath\cite{} & 0.602 ± 0.027 \\
& \mean & \underline{0.675 ± 0.022} \\
& $\ours$ & \textbf{0.778 ± 0.018} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.397 ± 0.025 \\
& \prism\cite{} & 0.601 ± 0.027 \\
& \gigapath\cite{} \mean & 0.497 ± 0.028 \\
& \gigapath\cite{} & 0.501 ± 0.023 \\
& \conch\cite{} \mean & \underline{0.614 ± 0.028} \\
& $\ours$ & \textbf{0.754 ± 0.019} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.657 ± 0.033 \\
& \gigapath\cite{} & 0.614 ± 0.027 \\
& $\ours$ Random Init & \underline{0.695 ± 0.022} \\
& $\ours$ & \textbf{0.733 ± 0.025} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_hnsc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-LSCC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{KEAP1 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{ARID1A Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & KEAP1 Mutation ($\uparrow$) (n=108) & ARID1A Mutation ($\uparrow$) (n=108) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & \underline{0.653 ± 0.018} & 0.535 ± 0.023 \\
& \prism\cite{} & 0.456 ± 0.018 & 0.548 ± 0.023 \\
& \gigapath\cite{} \mean & 0.583 ± 0.020 & 0.569 ± 0.022 \\
& \gigapath\cite{} & 0.576 ± 0.021 & \underline{0.590 ± 0.020} \\
& \mean & \textbf{0.669 ± 0.017} & 0.521 ± 0.020 \\
& $\ours$ & 0.646 ± 0.021 & \textbf{0.610 ± 0.027} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & \underline{0.671 ± 0.020} & 0.417 ± 0.020 \\
& \prism\cite{} & 0.491 ± 0.018 & 0.449 ± 0.020 \\
& \gigapath\cite{} \mean & 0.640 ± 0.017 & 0.437 ± 0.019 \\
& \gigapath\cite{} & 0.644 ± 0.018 & \underline{0.490 ± 0.017} \\
& \conch\cite{} \mean & 0.574 ± 0.018 & 0.411 ± 0.020 \\
& $\ours$ & \textbf{0.685 ± 0.019} & \textbf{0.658 ± 0.023} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.470 ± 0.023 & 0.469 ± 0.027 \\
& \gigapath\cite{} & \underline{0.613 ± 0.020} & \textbf{0.553 ± 0.019} \\
& $\ours$ Random Init & 0.601 ± 0.019 & 0.466 ± 0.018 \\
& $\ours$ & \textbf{0.614 ± 0.017} & \underline{0.508 ± 0.023} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_lscc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-LUAD\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{EGFR Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{STK11 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. \textbf{TP53 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|ccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{3}{c}{Tasks} \\ 
\cmidrule(lr){3-5}
& & EGFR Mutation ($\uparrow$) (n=108) & STK11 Mutation ($\uparrow$) (n=108) & TP53 Mutation ($\uparrow$) (n=108) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.710 ± 0.018 & 0.783 ± 0.023 & 0.618 ± 0.018 \\
& \prism\cite{} & 0.722 ± 0.016 & \underline{0.875 ± 0.015} & \underline{0.688 ± 0.016} \\
& \gigapath\cite{} \mean & 0.741 ± 0.018 & 0.814 ± 0.017 & 0.659 ± 0.019 \\
& \gigapath\cite{} & 0.723 ± 0.018 & 0.770 ± 0.022 & 0.631 ± 0.018 \\
& \mean & \underline{0.748 ± 0.017} & 0.810 ± 0.020 & 0.663 ± 0.016 \\
& $\ours$ & \textbf{0.767 ± 0.014} & \textbf{0.893 ± 0.015} & \textbf{0.722 ± 0.014} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.791 ± 0.015 & \underline{0.864 ± 0.013} & 0.735 ± 0.014 \\
& \prism\cite{} & \underline{0.809 ± 0.013} & 0.854 ± 0.015 & \textbf{0.756 ± 0.013} \\
& \gigapath\cite{} \mean & 0.782 ± 0.014 & 0.852 ± 0.013 & 0.715 ± 0.014 \\
& \gigapath\cite{} & 0.786 ± 0.014 & 0.827 ± 0.014 & 0.733 ± 0.013 \\
& \conch\cite{} \mean & 0.789 ± 0.014 & 0.824 ± 0.018 & 0.682 ± 0.015 \\
& $\ours$ & \textbf{0.822 ± 0.011} & \textbf{0.889 ± 0.015} & \underline{0.752 ± 0.014} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.761 ± 0.016 & 0.840 ± 0.015 & 0.671 ± 0.015 \\
& \gigapath\cite{} & 0.732 ± 0.015 & 0.812 ± 0.017 & 0.695 ± 0.017 \\
& $\ours$ Random Init & \textbf{0.809 ± 0.014} & \underline{0.869 ± 0.015} & \underline{0.719 ± 0.015} \\
& $\ours$ & \underline{0.792 ± 0.015} & \textbf{0.895 ± 0.011} & \textbf{0.758 ± 0.013} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_luad}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on CPTAC-PDAC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{SMAD4 Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & SMAD4 Mutation ($\uparrow$) (n=105) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.391 ± 0.017 \\
& \prism\cite{} & 0.593 ± 0.023 \\
& \gigapath\cite{} \mean & 0.260 ± 0.017 \\
& \gigapath\cite{} & 0.311 ± 0.020 \\
& \mean & \underline{0.606 ± 0.021} \\
& $\ours$ & \textbf{0.666 ± 0.022} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.488 ± 0.020 \\
& \prism\cite{} & 0.523 ± 0.022 \\
& \gigapath\cite{} \mean & 0.418 ± 0.020 \\
& \gigapath\cite{} & 0.426 ± 0.021 \\
& \conch\cite{} \mean & \underline{0.576 ± 0.020} \\
& $\ours$ & \textbf{0.578 ± 0.024} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.502 ± 0.019 \\
& \gigapath\cite{} & 0.331 ± 0.018 \\
& $\ours$ Random Init & \textbf{0.598 ± 0.021} \\
& $\ours$ & \underline{0.582 ± 0.022} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_cptac_pda}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on BRACS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Fine Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and standard error reported over 5-fold cross-validation. \textbf{Coarse Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=547) & Coarse Subtype ($\uparrow$) (n=547) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.275 ± 0.019 & 0.581 ± 0.039 \\
& \prism\cite{} & \textbf{0.474 ± 0.027} & \textbf{0.726 ± 0.020} \\
& \gigapath\cite{} \mean & 0.294 ± 0.021 & 0.567 ± 0.035 \\
& \gigapath\cite{} & 0.286 ± 0.018 & 0.575 ± 0.033 \\
& \mean & 0.336 ± 0.019 & 0.645 ± 0.020 \\
& $\ours$ & \underline{0.452 ± 0.024} & \underline{0.724 ± 0.028} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.348 ± 0.015 & 0.618 ± 0.028 \\
& \prism\cite{} & \underline{0.420 ± 0.015} & \underline{0.658 ± 0.019} \\
& \gigapath\cite{} \mean & 0.318 ± 0.016 & 0.569 ± 0.031 \\
& \gigapath\cite{} & 0.339 ± 0.018 & 0.608 ± 0.034 \\
& \conch\cite{} \mean & 0.377 ± 0.036 & 0.623 ± 0.036 \\
& $\ours$ & \textbf{0.481 ± 0.015} & \textbf{0.716 ± 0.019} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \textbf{0.504 ± 0.010} & 0.696 ± 0.031 \\
& \gigapath\cite{} & 0.459 ± 0.020 & 0.681 ± 0.020 \\
& $\ours$ Random Init & \underline{0.485 ± 0.019} & \textbf{0.757 ± 0.019} \\
& $\ours$ & 0.479 ± 0.022 & \underline{0.725 ± 0.019} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_bracs}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on eBRAINS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Fine Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. \textbf{Coarse Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=2319) & Coarse Subtype ($\uparrow$) (n=2319) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.557 ± TBD (0.000) & 0.713 ± TBD (0.000) \\
& \prism\cite{} & 0.624 ± TBD (0.000) & \underline{0.752 ± TBD (0.000)} \\
& \gigapath\cite{} \mean & \underline{0.626 ± TBD (0.000)} & 0.752 ± TBD (0.000) \\
& \gigapath\cite{} & 0.617 ± TBD (0.000) & 0.745 ± TBD (0.000) \\
& \mean & 0.549 ± TBD (0.000) & 0.724 ± TBD (0.000) \\
& $\ours$ & \textbf{0.705 ± TBD (0.000)} & \textbf{0.839 ± TBD (0.000)} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.704 ± TBD (0.000) & 0.871 ± TBD (0.000) \\
& \prism\cite{} & 0.714 ± TBD (0.000) & 0.872 ± TBD (0.000) \\
& \gigapath\cite{} \mean & \underline{0.738 ± TBD (0.000)} & \underline{0.901 ± TBD (0.000)} \\
& \gigapath\cite{} & 0.722 ± TBD (0.000) & 0.892 ± TBD (0.000) \\
& \conch\cite{} \mean & 0.693 ± TBD (0.000) & 0.874 ± TBD (0.000) \\
& $\ours$ & \textbf{0.741 ± TBD (0.000)} & \textbf{0.919 ± TBD (0.000)} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.722 ± TBD (0.000) & 0.882 ± TBD (0.000) \\
& \gigapath\cite{} & \textbf{0.747 ± TBD (0.000)} & \textbf{0.905 ± TBD (0.000)} \\
& $\ours$ Random Init & \textbf{0.747 ± TBD (0.000)} & \textbf{0.905 ± TBD (0.000)} \\
& $\ours$ & 0.741 ± TBD (0.000) & 0.895 ± TBD (0.000) \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_ebrains}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on IMPRESS-HER2\cite{huang2023artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{pCR}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & pCR ($\uparrow$) (n=62) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.487 ± 0.022 \\
& \prism\cite{} & \textbf{0.667 ± 0.022} \\
& \gigapath\cite{} \mean & 0.483 ± 0.020 \\
& \gigapath\cite{} & 0.601 ± 0.019 \\
& \mean & 0.474 ± 0.020 \\
& $\ours$ & \underline{0.611 ± 0.020} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.493 ± 0.019 \\
& \prism\cite{} & \textbf{0.642 ± 0.019} \\
& \gigapath\cite{} \mean & 0.495 ± 0.018 \\
& \gigapath\cite{} & 0.565 ± 0.022 \\
& \conch\cite{} \mean & 0.472 ± 0.019 \\
& $\ours$ & \underline{0.603 ± 0.020} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.701 ± 0.022} \\
& \gigapath\cite{} & 0.533 ± 0.018 \\
& $\ours$ Random Init & 0.531 ± 0.019 \\
& $\ours$ & \textbf{0.709 ± 0.019} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_impress_her2}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on IMPRESS-TNBC\cite{huang2023artificial} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{pCR}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & pCR ($\uparrow$) (n=64) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & \underline{0.639 ± 0.020} \\
& \prism\cite{} & 0.587 ± 0.021 \\
& \gigapath\cite{} \mean & 0.594 ± 0.020 \\
& \gigapath\cite{} & 0.598 ± 0.020 \\
& \mean & 0.570 ± 0.022 \\
& $\ours$ & \textbf{0.657 ± 0.020} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & \underline{0.665 ± 0.017} \\
& \prism\cite{} & 0.541 ± 0.017 \\
& \gigapath\cite{} \mean & \textbf{0.669 ± 0.018} \\
& \gigapath\cite{} & 0.617 ± 0.018 \\
& \conch\cite{} \mean & 0.652 ± 0.020 \\
& $\ours$ & 0.602 ± 0.021 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.615 ± 0.020} \\
& \gigapath\cite{} & 0.595 ± 0.021 \\
& $\ours$ Random Init & \textbf{0.644 ± 0.020} \\
& $\ours$ & 0.604 ± 0.022 \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_impress_tnbc}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on OV-Bevacizumab\cite{wang2022weakly} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Response}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=36) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.740 ± 0.026 \\
& \prism\cite{} & 0.443 ± 0.041 \\
& \gigapath\cite{} \mean & 0.733 ± 0.027 \\
& \gigapath\cite{} & 0.760 ± 0.028 \\
& \mean & \underline{0.797 ± 0.026} \\
& $\ours$ & \textbf{0.857 ± 0.025} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.607 ± 0.033 \\
& \prism\cite{} & 0.433 ± 0.034 \\
& \gigapath\cite{} \mean & 0.523 ± 0.034 \\
& \gigapath\cite{} & 0.603 ± 0.039 \\
& \conch\cite{} \mean & \underline{0.623 ± 0.030} \\
& $\ours$ & \textbf{0.863 ± 0.021} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.540 ± 0.033 \\
& \gigapath\cite{} & 0.457 ± 0.046 \\
& $\ours$ Random Init & \underline{0.753 ± 0.028} \\
& $\ours$ & \textbf{0.780 ± 0.032} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_ovarian}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on NADT Prostate\cite{wilkinson2021nascent} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Response}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=36) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.695 ± 0.023 \\
& \prism\cite{} & \textbf{0.752 ± 0.024} \\
& \gigapath\cite{} \mean & 0.668 ± 0.027 \\
& \gigapath\cite{} & 0.688 ± 0.026 \\
& \mean & 0.683 ± 0.022 \\
& $\ours$ & \underline{0.725 ± 0.023} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.612 ± 0.027 \\
& \prism\cite{} & \underline{0.720 ± 0.023} \\
& \gigapath\cite{} \mean & 0.585 ± 0.028 \\
& \gigapath\cite{} & 0.577 ± 0.024 \\
& \conch\cite{} \mean & 0.622 ± 0.026 \\
& $\ours$ & \textbf{0.730 ± 0.022} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.583 ± 0.033 \\
& \gigapath\cite{} & 0.525 ± 0.036 \\
& $\ours$ Random Init & \textbf{0.717 ± 0.022} \\
& $\ours$ & \underline{0.702 ± 0.020} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_nadt}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on GBM-Treatment\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Response}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Response ($\uparrow$) (n=93) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.642 ± 0.019 \\
& \prism\cite{} & 0.633 ± 0.019 \\
& \gigapath\cite{} \mean & 0.633 ± 0.019 \\
& \gigapath\cite{} & \textbf{0.672 ± 0.016} \\
& \mean & \underline{0.668 ± 0.018} \\
& $\ours$ & 0.659 ± 0.018 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.580 ± 0.018 \\
& \prism\cite{} & 0.622 ± 0.022 \\
& \gigapath\cite{} \mean & 0.605 ± 0.017 \\
& \gigapath\cite{} & 0.618 ± 0.017 \\
& \conch\cite{} \mean & \underline{0.703 ± 0.018} \\
& $\ours$ & \textbf{0.741 ± 0.016} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.704 ± 0.018} \\
& \gigapath\cite{} & 0.642 ± 0.017 \\
& $\ours$ Random Init & 0.660 ± 0.018 \\
& $\ours$ & \textbf{0.707 ± 0.016} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_gbm_rt_tmz}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on Post-NAT-BRCA\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Lymphovascular Invasion}: This is a slide-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|c}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{1}{c}{Tasks} \\ 
\cmidrule(lr){3-3}
& & Lymphovascular Invasion ($\uparrow$) (n=53) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.594 ± 0.026 \\
& \prism\cite{} & 0.487 ± 0.024 \\
& \gigapath\cite{} \mean & \underline{0.625 ± 0.027} \\
& \gigapath\cite{} & \textbf{0.627 ± 0.025} \\
& \mean & 0.568 ± 0.026 \\
& $\ours$ & 0.601 ± 0.027 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.612 ± 0.028 \\
& \prism\cite{} & 0.540 ± 0.029 \\
& \gigapath\cite{} \mean & 0.603 ± 0.025 \\
& \gigapath\cite{} & 0.577 ± 0.024 \\
& \conch\cite{} \mean & \underline{0.654 ± 0.022} \\
& $\ours$ & \textbf{0.701 ± 0.027} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.553 ± 0.025 \\
& \gigapath\cite{} & \underline{0.615 ± 0.025} \\
& $\ours$ Random Init & 0.580 ± 0.023 \\
& $\ours$ & \textbf{0.662 ± 0.028} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_natbrca}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on SURGEN\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{BRAF Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{RAS Mutation}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{MMR Loss}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. \textbf{Death in 5 Years}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 5-fold cross-validation. }
\scalebox{0.675}{\begin{tabular}{ll|cccc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{4}{c}{Tasks} \\ 
\cmidrule(lr){3-6}
& & BRAF Mutation ($\uparrow$) (n=388) & RAS Mutation ($\uparrow$) (n=389) & MMR Loss ($\uparrow$) (n=389) & Death in 5 Years ($\uparrow$) (n=387) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.599 ± 0.037 & 0.584 ± 0.034 & 0.739 ± 0.057 & 0.627 ± 0.023 \\
& \prism\cite{} &  &  &  &  \\
& \gigapath\cite{} \mean & 0.629 ± 0.029 & 0.616 ± 0.019 & 0.794 ± 0.040 & 0.636 ± 0.022 \\
& \gigapath\cite{} & 0.616 ± 0.021 & 0.618 ± 0.010 & 0.779 ± 0.046 & 0.631 ± 0.024 \\
& \mean & \underline{0.641 ± 0.020} & \underline{0.619 ± 0.020} & \underline{0.819 ± 0.026} & \underline{0.663 ± 0.023} \\
& $\ours$ & \textbf{0.753 ± 0.039} & \textbf{0.649 ± 0.029} & \textbf{0.914 ± 0.019} & \textbf{0.667 ± 0.017} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.693 ± 0.037 & 0.586 ± 0.030 & \underline{0.880 ± 0.017} & 0.642 ± 0.021 \\
& \prism\cite{} &  &  &  &  \\
& \gigapath\cite{} \mean & \underline{0.694 ± 0.033} & 0.605 ± 0.015 & 0.877 ± 0.017 & \underline{0.663 ± 0.016} \\
& \gigapath\cite{} & 0.679 ± 0.026 & 0.621 ± 0.022 & 0.861 ± 0.015 & 0.633 ± 0.013 \\
& \conch\cite{} \mean & 0.649 ± 0.025 & \underline{0.630 ± 0.028} & 0.797 ± 0.037 & 0.661 ± 0.023 \\
& $\ours$ & \textbf{0.726 ± 0.042} & \textbf{0.632 ± 0.027} & \textbf{0.910 ± 0.023} & \textbf{0.685 ± 0.017} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & 0.692 ± 0.046 & \underline{0.656 ± 0.017} & 0.841 ± 0.035 & 0.695 ± 0.017 \\
& \gigapath\cite{} &  &  &  &  \\
& $\ours$ Random Init & \underline{0.715 ± 0.032} & 0.635 ± 0.026 & \underline{0.893 ± 0.030} & \underline{0.703 ± 0.029} \\
& $\ours$ & \textbf{0.798 ± 0.031} & \textbf{0.675 ± 0.014} & \textbf{0.894 ± 0.035} & \textbf{0.733 ± 0.024} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_sr386_}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on MBC\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Recist}: This is a patient-level classification task evaluated using quadratic weighted kappa, mean and standard error reported over 50-fold Monte Carlo. \textbf{Recist Binary}: This is a patient-level classification task evaluated using AUROC, mean and standard error reported over 50-fold Monte Carlo. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Recist ($\uparrow$) (n=76) & Recist Binary ($\uparrow$) (n=76) \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean & 0.149 ± 0.030 & 0.666 ± 0.018 \\
& \prism\cite{} & \underline{0.232 ± 0.035} & 0.631 ± 0.018 \\
& \gigapath\cite{} \mean & 0.098 ± 0.033 & \textbf{0.681 ± 0.019} \\
& \gigapath\cite{} & 0.129 ± 0.035 & 0.665 ± 0.019 \\
& \mean & 0.181 ± 0.036 & \underline{0.671 ± 0.019} \\
& $\ours$ & \textbf{0.233 ± 0.034} & 0.624 ± 0.018 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean & 0.050 ± 0.028 & 0.560 ± 0.017 \\
& \prism\cite{} & 0.206 ± 0.034 & 0.583 ± 0.020 \\
& \gigapath\cite{} \mean & 0.131 ± 0.034 & 0.580 ± 0.018 \\
& \gigapath\cite{} & 0.047 ± 0.034 & 0.558 ± 0.018 \\
& \conch\cite{} \mean & \underline{0.253 ± 0.038} & \textbf{0.639 ± 0.019} \\
& $\ours$ & \textbf{0.258 ± 0.037} & \underline{0.609 ± 0.015} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \underline{0.315 ± 0.040} & \underline{0.668 ± 0.018} \\
& \gigapath\cite{} &  &  \\
& $\ours$ Random Init &  &  \\
& $\ours$ & \textbf{0.350 ± 0.035} & \textbf{0.675 ± 0.017} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:normal_mbc_}
\end{table}


\begin{table}[h]
\centering
\caption{\textbf{WITH RANDOMINIT Performance comparison between $\ours$ and baselines on eBRAINS\cite{} tasks.} Best in \textbf{bold}, second best is \underline{underlined}. \textbf{Fine Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. \textbf{Coarse Subtype}: This is a slide-level classification task evaluated using balanced accuracy, mean and 95\% CI reported over 100 bootstraps of a single fold. }
\scalebox{0.675}{\begin{tabular}{ll|cc}
\toprule
 & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Tasks} \\ 
\cmidrule(lr){3-4}
& & Fine Subtype ($\uparrow$) (n=2319) & Coarse Subtype ($\uparrow$) (n=2319) \\
\midrule
\multirow{8}{*}{\rotatebox{90}{\scriptsize{\textbf{ProtoNet}}}}
& \virchow\cite{} \mean &  &  \\
& \prism\cite{} &  &  \\
& \gigapath\cite{} \mean &  &  \\
& \gigapath\cite{} &  &  \\
& \chief\cite{} \mean & \textbf{0.490 (0.451-0.534)} & \textbf{0.602 (0.541-0.650)} \\
& \chief\cite{} & \underline{0.424 (0.383-0.462)} & \underline{0.474 (0.412-0.520)} \\
& \conch\cite{} \mean &  &  \\
& $\ours$ &  &  \\
\midrule
\multirow{8}{*}{\rotatebox{90}{\scriptsize{\textbf{Linear Probe}}}}
& \virchow\cite{} \mean &  &  \\
& \prism\cite{} &  &  \\
& \gigapath\cite{} \mean &  &  \\
& \gigapath\cite{} &  &  \\
& \chief\cite{} \mean & \textbf{0.639 (0.591-0.678)} & \textbf{0.780 (0.731-0.828)} \\
& \chief\cite{} & \underline{0.582 (0.534-0.624)} & \underline{0.740 (0.695-0.791)} \\
& \conch\cite{} \mean &  &  \\
& $\ours$ &  &  \\
\midrule
\multirow{4}{*}{\rotatebox{90}{\scriptsize{\textbf{Supervised}}}}
& ABMIL & \textbf{} & \textbf{} \\
& \gigapath\cite{} & \textbf{} & \textbf{} \\
& $\ours$ Random Init & \textbf{} & \textbf{} \\
& $\ours$ & \textbf{} & \textbf{} \\
\midrule
\bottomrule
\end{tabular}
}\label{tab:allshot_ebrains}
\end{table}

